Efficiently Sampling and Estimating from Substructures using Linear Algebraic Queries

Given an unknown $n \times n$ matrix $A$ having non-negative entries, the \emph{inner product} (IP) oracle takes as inputs a specified row (or a column) of $A$ and a vector $v \in \mathbb{R}^{n}$, and returns their inner product. A derivative of IP is the induced degree query in an unknown graph $G=(V(G), E(G))$ that takes a vertex $u \in V(G)$ and a subset $S \subseteq V(G)$ as input and reports the number of neighbors of $u$ that are present in $S$. The goal of this paper is to understand the strength of the inner product oracle. Our results in that direction are as follows: (I) IP oracle can solve bilinear form estimation, i.e., estimate the value of ${\bf x}^{T}A\bf{y}$ given two vectors ${\bf x},\, {\bf y} \in \mathbb{R}^{n}$ with non-negative entries and can sample almost uniformly entries of a matrix with non-negative entries; (ii) We tackle for the first time weighted edge estimation and weighted sampling of edges that follow as an application to the bilinear form estimation and almost uniform sampling problems, respectively; (iii) induced degree query, a derivative of IP can solve edge estimation and an almost uniform edge sampling in induced subgraphs. To the best of our knowledge, these are the first set of Oracle-based query complexity results for induced subgraphs. We show that IP/induced degree queries over the whole graph can simulate local queries in any induced subgraph; (iv) Apart from the above, we also show that IP can solve several problems related to matrix, like testing if the matrix is diagonal, symmetric, doubly stochastic, etc.

==> append.tex <==
\input{color-upper.tex}
%\input{other-upper.tex}
%\input{color-lower.tex}

%\section{Algorithm for \conflictest in \varand model}\label{sec:est-rand-algo}
%%%%%Algorithm for \conflictest in \varand model

\begin{algorithm}[h]
%\scriptsize

\LinesNumbered

\caption{{\sc Random-Order-Est}($\vareps,T)$: \conflictest in \varandlong model}
\label{algo:random-order}
\KwIn{$G = (V, E)$ and a coloring function $f$ on $V$ in the \varand model, parameters $T$ and $\vareps$.}
\KwOut{$\hat{m}$, that is, a $(1\pm \vareps)$ approximation to $\size{E_M}$.}
%Initialize $\hat{m_h}=0$\.\
Set $t = \lceil \log _{1+\frac{\vareps}{10}}n \rceil$. If $T <63t^2$, then store all the vertices in $G$ along with their colors. At the end, 
report the exact value of $\size{E_M}$. Otherwise, we proceed as follows.\\ 
Let 
\begin{itemize}
\item $\Gamma=\widetilde{\Theta} \left( \frac{n}{\sqrt{T}}\right)$;
\item $v_1,\ldots,v_n$ be the random ordering in which vertices are revealed and $R=\{v_1,\ldots,v_\Gamma\}$;
\item  $\kappa_i, i \in [n],$ denotes the number of monochromatic neighbors of $v_i$ in $R$, that is, 
$\kappa_i = \size{\{(u,v_i): u \in R~\mbox{and}~f(u)=f(v_i)\}}$.
\item $\hat{d_i}, i \in [n],$ denotes the (estimated) monochromatic neighbors of vertices in $G$.\\
\item $H$ denotes the set of \emph{high} degree vertex in $R$, that is, $H=\{v_i:\kappa_i \geq \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8t}\}$
and $L=V \setminus H$;  $L_R=L \cap R$ and $H_R=H \cap R$;
\item The vertices in $L$ are partitioned into $t$ buckets as follows:\\
$B_j=\{v_i \in L: \left(1+\frac{\vareps}{10} \right)^{j-1} \leq d_M(v_i) < \left(1+\frac{\vareps}{10}\right)^{j} \}$, where $j \in [t]$.\\

\end{itemize}

\For{(for each vertex $v_i \in R$ exposed in the stream)}
{
Store $v_i$ as well as its color $f(v_i)$.\\
For each edge $(v_{i'},v_i)$ that arrives in the stream, increase the values of $\kappa_{i'}$ and $\kappa_i$.\\
}
\For{(each $v_i \in R$ with $\kappa_i \geq  \frac{ \size{R}}{n}\frac{\sqrt{\vareps T}}{8t}$)}
{
Add $v_i$ to $H_R$. \\ 
Set $\widehat{d_i}=\frac{n}{\size{R}}\kappa_i$.\\
}
$\widehat{m_h}=\sum\limits_{v_i \in H} \widehat{d_i}$.\\
Let $L_R = R \setminus H_R$. \\
\For{(each $v_i \in L_R$)}
{
Set $\widehat{d_i}=\kappa_i$.\\
}
\For{(for each vertex $v_i \notin R$ exposed in the stream)}
{
Determine the value of $\kappa_i$. If $\kappa_i \geq  \frac{ \size{R}}{n}\frac{\sqrt{\vareps T}}{8t}$, find $\widehat{d_i}=\frac{n}{\size{R}}\kappa_i$ and add $\widehat{d_i}$ to the current $\widehat{m_h}.$ \\
Also, for each $v_{i'} \in L_R$, increase the value of $\widehat{d_{i'}}$ if $(v_{i'},v_i)$ is an edge.\\
}
From the values of $\widehat{d_i}$ for all $v_i \in L_R$, determine the buckets for each vertex in $L_R$. Also, for each $j \in [t]$, find the set $ A_j=\size{L_R \cap B_j}$. Then determine $$\widehat{m_\ell}=\frac{n}{\size{R}}\sum\limits_{ j \in [t]} \size{A_j} \left(1+\frac{\vareps}{10}\right)^i .$$\\
Report $\widehat{m}=\frac{m_h+m_\ell}{2}$ as the final {\sc Output}.
\end{algorithm}


\section{Some probability results}\label{sec:prob}
\begin{lemma}[\cite{DBLP:journals/eatcs/Mulzer18}] \label{lem:without-replace}
Let $I=\{1,\ldots,N\}$, $r \in [N]$ be a given parameter. If we sample a subset $R$ with replacement, then the following holds for any $J \subset I$ and $\delta \in (0,1)$.
\begin{itemize}
\item[(i)] $\pr \left( \size{J \cap R} \geq (1+\delta)\size{J}\frac{r}{N}\right) \leq \exp{\left(-\frac{\delta^2\size{J}r}{3N}\right)}$;
\item[(ii)] $\pr \left( \size{J \cap R} \leq (1-\delta)\size{J}\frac{r}{N}\right) \leq \exp{\left(-\frac{\delta^2\size{J}r}{3N}\right)}$;
\item[(iii)] Further more, we have the following if $\size{J} \leq k$, then the following holds.
 \[\pr \left( \size{J \cap R} \geq (1+\delta)k\frac{r}{N}\right) \leq \exp{\left(-\frac{\delta^2kr}{3N}\right)}\]
\end{itemize}

\end{lemma}

\begin{lemma}[\cite{DBLP:books/daglib/0025902}(Chernoff-Hoeffding bound)]
\label{lem:cher_bound1}
Let $X_1, \ldots, X_n$ be independent random variables such that $X_i \in [0,1]$. For $X=\sum\limits_{i=1}^n X_i$ and $\mu=\mathbb{E}[X]$, the following holds for any $0 \leq \delta \leq 1$:
\[ \mathbb{P}(|X - \mu| \geq \delta\mu) \leq 2\exp{\left( \frac{-\mu \delta^{2}}{3}\right)} \]
\end{lemma}

\remove{
\begin{lemma}[\cite{DBLP:books/daglib/0025902}(Chernoff-Hoeffding bound)]
\label{lem:cher_bound2}
Let $X_1, \ldots, X_n$ be independent random variables such that $X_i \in [0,1]$. For $X=\sum\limits_{i=1}^n X_i$ and $\mu_l \leq \mathbb{E}[X] \leq \mu_h$, the following holds for any $\delta >0$.
\begin{romanenumerate}
\item $\mathbb{P} \left( X \geq \mu_h + \delta \right) \leq \exp{\left(\frac{-2\delta^2}{n}\right)}$
\item $\mathbb{P} \left( X \leq \mu_l - \delta \right) \leq \exp{\left(\frac{-2\delta^2}{n}\right)}$
\end{romanenumerate}
\end{lemma}

\begin{lemma}[Theorem 3.2 in~\cite{DBLP:books/daglib/0025902}]
\label{lem:depend:high_exact_statement}
Let $X_1,\ldots,X_n$ be random variables such that $a_i \leq X_i \leq b_i$ and $X=\sum\limits_{i=1}^n X_i$. Let $\mathcal{D}$ be the \emph{dependent} graph, where $V(\mathcal{D})=\{X_1,\ldots,X_n\}$ and $ E(\mathcal{D})= \{(X_i,X_j): \mbox{$X_i$ and $X_j$ are dependent}\}$. Then for any $\delta >0$, 
\[ \mathbb{P}(|X-\mathcal{E}[X]| \geq \delta) \leq  2e^{\frac{-2\delta^2}{\chi^*(\mathcal{D})\sum\limits_{i=1}^{n}(b_i-a_i)^2}} \]
where $\chi^*(\mathcal{D})$ denotes the \emph{fractional chromatic number} of $\mathcal{D}$.
\end{lemma}

The following lemma directly follows from Lemma~\ref{lem:depend:high_exact_statement}
\begin{lemma}[Chernoff bound for bounded dependency]
\label{lem:depend:high_prob}
Let $X_1,\ldots,X_n$ be indicator random variables such that there are at most $d$ many $X_j$'s on which an $X_i$ depends. For $X=\sum\limits_{i=1}^n X_i$ and $\mu_l \leq \mathbb{E}[X] \leq \mu_h$, the following holds for any $\delta >0$:
\begin{romanenumerate}
\item $\mathbb{P}(X \geq \mu_h + \delta) \leq e^{\frac{-2\delta^2}{(d+1)n}}$
\item $\mathbb{P}(X-\mu_\ell  \leq \delta) \leq e^{\frac{-2\delta^2}{(d+1)n}}$
\end{romanenumerate}
\end{lemma}
}

\section{Communication Complexity}\label{sec:comm}

Communication Complexity~\cite{DBLP:books/daglib/0011756} deals with finding the minimum amount of space that is needed to communicate in order to compute a function when the input to the function is distributed among multiple parties. For the purpose of our work, we are concerned with two player games with one-way communication protocol. The players are traditionally called Alice and Bob. Both of them have a $n$-bit input string and are unaware of each other's input. The goal is to minimize the bits Alice needs to communicate to Bob so that he can compute a function on both their inputs. No assumption is made on their computational powers and there is no restriction on the amount of time needed for computing the function. 

%%%%%%%%%modify
\subsection{INDEX problem in the communication complexity model}

Lower bound results in the streaming model of computation are proved by reduction from a problem in communication complexity model. We determine our lower bounds by considering a reduction from the INDEX problem in the one-way communication protocol for two players to the specific problem in graphs in the \va model. The INDEX problem is defined as follows:
There are two parties, Alice and Bob. Alice has a $N$-bit input string $X \in \{0,1\}^{N}$ and Bob has an integer $j \in [N]$. Both are unaware of each other's input and the goal is to compute $X_{j}$, the $j^{th}$ bit of $X$. The lower bound for space complexity to solve the INDEX problem in the one-way deterministic communication model is $\Omega(N)$. 
\begin{lemma}\label{index}
The deterministic communication complexity of INDEX is $\Omega(N)$
\end{lemma}

\remove{
\begin{algorithm}[h]
\SetAlgoLined
\caption{{\sc VA-DegreeOracle-Sep}}
\label{algo:deg-oracle}
\KwIn{$G = (V, E)$ and a coloring function $f$ on $V$ in the \vadeg model}
\KwOut{The algorithm verifies if $f$ is $\vareps$-far from valid or not}

\texttt{Initialize a reservoir } $R$ \texttt{ of size } $t$ \\
    \For{$i \gets 1$ \texttt{ to } $|V|$} { %\comment{loop through the vertices in the stream}
       \texttt{let } $u$ \texttt{ be the } $i^{th}$ \texttt{ vertex of the stream and } $d_{G}(u)$ \texttt{ be its degree}
        \For{$j \gets 1$ \texttt{ to } $t$} { %\comment{loop through the stored vertices in the reservoir}
            \If{$u$ \texttt{ is adjacent to the } $j^{th}$ \texttt{ vertex } $v$ \texttt{ stored in } $R$} {
                \texttt{increment the value of } $v's$ \texttt{ count by } $1$ \\
                \If{$count$ \texttt{ is } $b$ \texttt{(i.e., } $u$ \texttt{ is } $v's$ $b^{th}$ \texttt{ successive neighbor in the stream)} }  {
                    \texttt{store } $u$ \texttt{, along with its color } $f(u)$ \texttt{, as the} $b^{th}$ \texttt{ neighbor of } $v$ \texttt{ (equivalent to storing the edge } $(u,v)$ \texttt{ with their respective colors } $f(u)$ \texttt{ and } $f(v)$ \texttt{ to check if it is monochromatic or not)}
                 }
            }
        %loop through the vertices stored in reservoir R
       }
    %\COMMENT{loop through vertices of the stream}
        \If{$i \leq t$} {
        \texttt{store } $u$ \texttt{ and its color } $f(u)$ \texttt{ and initialize its count to } $0$ \\
        $d^{+}_{G}(u) \gets d_{G}(u) - d^{-}_{G}(u) $ \\
        \texttt{choose } $b$ \texttt{ uniformly at random in the range } $[d^{+}_{G}(u)]$
        }
    	\Else {
        \texttt{with probability } $\frac{t}{i}$ \texttt{, replace an element of the reservoir } $R$ \texttt{, chosen uniformly at random, with } $u$ \texttt{ and its color } $f(u)$ \\
        \texttt{initialize } $u's$ \texttt{ count to } $0$ \\
        \texttt{choose } $b$ \texttt{ uniformly at random from } $[d^{+}_{G}(u)]$ \texttt{(and replace the previous vertex's neighbor, if it has been stored)}
    	}
  }
  \For{$i \gets 1$ \texttt{ to } $t$} {
        \texttt{let } $u$ \texttt{ be the } $i^{th}$ \texttt{ vertex stored in the reservoir } $R$ \texttt{ and } $v$ \texttt{ its stored neighbor (with their respective colors)} \\
        \texttt{check if the assigned the colors to } $u$ \texttt{ and } $v$ \texttt{ make the edge } $(u,v)$ \texttt{ monochromatic}
    }
  \caption{Algorithm: \colorverify in \vadeglong model}
\end{algorithm}
}




==> color-lower.tex <==
\section{Lower bounds for \colorverify} \label{sec:sep-valb}

We show a tight lower bound of $\Omega(\frac{1}{\epsilon})$ for the \colorverify problem in the vertex arrival model with degree oracle. For the \colorverify problem in the vertex arrival model we show a tight lower bound of $\Omega(\frac{|V|}{\sqrt |E|})$. These bounds are proved using reductions from the \emph{INDEX} problem in the one-way communication complexity model to the \colorverify problem in graphs in the vertex arrival model. In the INDEX problem, Alice gets an $M$-bit string $X\in \{0,1\}^M$ and Bob gets an integer $j\in [M]$. Both Alice and Bob are unaware of each other's input. Alice can send a message to Bob and Bob has to output $X_j$. It is well known that the lower bound on the message length for the INDEX problem in the one-way communication complexity model is $\Omega(M)$ (See Lemma~\ref{index} in Appendix~\ref{sec:comm}).

\subsection{Lower bound for \colorverify in \vadeg model} \label{sec:sep-vadglbsc}

\begin{theorem}\label{theo:sep-vadglbth}
The lower bound for the \colorverify problem in the \vadeg streaming model is $\Omega(\frac{1}{\vareps})$.
\end{theorem}

\begin{proof}
%To determine the lower bound, we consider a reduction from the INDEX problem in the one-way communication protocol to the \colorverify problem in graphs in the \va model with the degree oracle. 

We show the lower bound using a reduction from the INDEX problem in one-way communication complexity to the \colorverify problem in graphs in the vertex arrival model with access to degree oracle. The reduction works as follows: For each input bit $X_i$, Alice constructs a bipartite graph with bipartition $(L_i,R_i)$, where $L_i$ and $R_i$ are independent sets of size $k$. For any two sets $L_s$ and $R_t$, Alice does not add any edge between vertices in $L_s$ and $R_t$. If $X_i$ equals $1$, then vertices in $L_i$ are colored with color $C_1$, else they are colored with color $C_0$. At the end of the stream, Alice sends this memory state to Bob. Bob colors all vertices in $R_i$ for $1\leq i\neq j \leq M$ with color $C_2$. Vertices in $R_j$ are colored with $C_1$. Moreover, for any index $i\in [M]$, Bob adds all edges between $L_i$ and $R_i$. Access to a degree oracle does not provide any advantage to any protocol on this instance. The only difference is in the construction of the graph.
Now, if $X_j=0$, then there are no monochromatic edges in the graph. However, if $X_j=1$, there are $k^2$ monochromatic edges. The number of vertices in the graph is $n=Mk$ and the number of edges is $m=Mk^2$. The number of conflicting edges in the graph is $k^{2}= \vareps m=\vareps Mk^{2}$.
Therefore, for $M=\frac{1}{\eps}$, distinguishing whether the graph is properly-colored (valid) or at least $\eps$-fraction of edges are monochromatic ($\eps$-far from being valid) requires $\Omega(\frac{1}{\eps})$ space.

%Alice has a $M$-bit input string $X \in \{0,1\}^{M}$ and Bob has an integer $j \in [M]$. The lower bound for space complexity to solve the INDEX problem in the one-way communication model is $\Omega(M)$ [Lemma~\ref{index}]. We consider the stream of vertices $X_{1}, X_{2}, ..., X_{M}$ arriving in an arbitrary order as the input to Alice. For each $X_{i}$, we associate a bipartite graph gadget with it. Each partition consists of k vertices and we denote the left and right partitions as $L_{i}$ and $R_{i}$ respectively. $L_{i}$ and $R_{i}$, $\forall i \in [M]$, are independent sets. When Alice receives the bit $X_{i}$, she colors the vertices of $L_{i}$ with the color $C_{0}$, if $X_{i} = 0$, else, she colors the vertices of $L_{i}$ with the color $C_{1}$, if $X_{i} = 1$. Alice saves this memory state and sends it to Bob. Bob colors all the vertices of  $R_{i}$ with the color $C_{2}$, $\forall i \in [M]$, $i \neq j$. However, for the index $j$, he colors all the vertices of $R_{j}$ with color $C_{1}$.  $\forall i \in [M]$, Bob adds all the edges to the gadget for $X_{i}$ to make it a complete bipartite graph. If $X_{j} = 0$, then the color of $L_{j}$ is $C_{0}$ and there are no conflicting edges, whereas if $X_{j} = 1$, then the color of $L_{j}$ is $C_{1}$ and there will be $k^{2}$ conflicting edges. The number of vertices in the graph, $n$, is $\Theta(Mk)$ while the number of edges in the graph, $m$, is $\Theta(Mk^{2})$ and the number of conflicts in the graph is $k^{2}$.
%\[ k^{2} =  \vareps m = \vareps Mk^{2} \] \[ M = \Omega(\frac{1}{\vareps}) \]
\end{proof}

\subsection{Lower bound for \colorverify in \va model} \label{sec:sep-vaaolbsc}

\begin{theorem}\label{theo:sep-vaaolbth} The space lower bound for the \colorverify problem in the \va model is $\Omega\left(\frac{|V|}{\sqrt{|E|}}\right)$. \end{theorem}

\begin{proof} We show the lower bound using a reduction from the INDEX problem in one-way communication complexity to the \colorverify problem in graphs in the order vertex arrival model. For each input bit $X_i$, Alice constructs a bipartite graph with bipartition $(L_i,R_i)$, where $L_i$ and $R_i$ are independent sets of size $k$. For any two sets $L_s$ and $R_t$, Alice does not add any edge between vertices in $L_s$ and $R_t$. If $X_i$ equals $1$, then vertices in $L_i$ are colored with color $C_1$, else they are colored with color $C_0$. At the end of the stream, Alice sends this memory state to Bob. Bob colors all vertices in $R_i$ for $1\leq i\leq M$ with color $C_1$. Moreover, for index $j$, he adds all the edges between $L_j$ and $R_j$ to make it a complete bipartite graph. Now, if $X_j=0$, then there are no monochromatic edges. However, if $X_j=1$, there are $k^2$ monochromatic edges. We have the number of vertices in the graph $n=Mk$ and the number of edges $m=k^2$. Therefore, for $M=\frac{n}{\sqrt{m}}$ or $\frac{|V|}{\sqrt{|E|}}$, distinguishing whether the graph is properly-colored (valid) or all of its edges are monochromatic ($\eps$-far from being valid) requires $\Omega\left(\frac{|V|}{\sqrt{|E|}}\right)$ space.


%To determine the lower bound, we consider a reduction from the INDEX problem in the one-way communication protocol to the \colorverify problem in graphs in the arbitrary order \va model.

%Alice has a $M$-bit input string $X \in \{0,1\}^{M}$ and Bob has an integer $j \in [M]$. The lower bound for space complexity to solve the INDEX problem in the one-way communication model is $\Omega(M)$ [Lemma~\ref{index}]. 
%We consider the stream of vertices $X_{1}, X_{2}, ..., X_{M}$ arriving in an arbitrary order as the input to Alice. For each $X_{i}$, we associate a bipartite graph gadget with it. Each partition consists of k vertices and we denote the left and right partitions as $L_{i}$ and $R_{i}$ respectively. $L_{i}$ and $R_{i}$, $\forall i \in [M]$, are independent sets. When Alice receives the bit $X_{i}$, she colors the vertices of $L_{i}$ with the color $C_{0}$, if $X_{i} = 0$, else, she colors the vertices of $L_{i}$ with the color $C_{1}$, if $X_{i} = 1$. Alice saves this memory state and sends it to Bob. Bob colors all the vertices of  $R_{i}$ with the color $C_{1}$, $\forall i \in [M]$. However, for the index $j$, he adds all the edges to the gadget for $X_{j}$ to make it a complete bipartite graph. If $X_{j} = 0$, then the color of $L_{j}$ is $C_{0}$ and there are no conflicting edges, whereas if $X_{j} = 1$, then the color of $L_{j}$ is $C_{1}$ and there will be $k^{2}$ conflicting edges. The number of vertices in the graph, $n$, is $\Theta(Mk)$ while the number of edges in the graph, $m$, is $\Theta(k^{2})$. Given $n$ and $m$, we can set the values of $M$ and $k$ accordingly.
%\[ k ={\sqrt m} \] \[ M = \Omega(\frac{n}{\sqrt m}) \]
\end{proof}



==> color-upper.tex <==
\section{\colorverify in \varand model} \label{sec:sep-vaub}

%\subsection{\colorverify in \varand model} \label{sec:sep-vardubsc}

We solve the \colorverify problem for graphs in the vertex arrival model when vertices stream in a random order.

\begin{theorem}\label{thm:sep-vardubth} 
Given any graph $G=(V,E)$ and a coloring function $f:V(G) \rightarrow [C]$ and a parameter $\vareps>0$ as input, there exists an algorithm that solves the \colorverify problem in the \varand streaming model using space $ \widetilde{\mathcal{O}} \left(\frac{\size{V}}{\sqrt{\vareps \size{E}}} \right)$ with high probability. \end{theorem}


Let $G'$ denote the subgraph of $G$ consisting of only monochromatic edges in $G$. The lemma stated below guarantees that either there exists a large matching of size at least $\sqrt{\eps m}$ in $G'$ or there exists a vertex of degree at least $\sqrt{\eps m}$ in $G'$.
\remove{ \comments{Include the reference for the following lemma}}

\begin{lemma}[\cite{DBLP:series/txtcs/Jukna11}]\label{lem:sunflower} Let $G=(V,E)$ be a graph and $f:V(G) \rightarrow [C]$ be a coloring function such that at least $\vareps$ fraction of the edges $E(G)$ known to be monochromatic. Then, either there is a matching of size at least $\sqrt{\vareps m}$ or there exists a vertex of degree at least $\sqrt{\vareps m}$ in the subgraph $G'$ defined on the monochromatic edges of $G$. \end{lemma}

The algorithm works as follows. We sample independently and uniformly at random the vertices in stream with probability $p=\min\{1,\frac{10\log n}{\sqrt{m}}\}$ \remove{\footnote{\comments{What if $\frac{c\log n}{\sqrt{m}}\geq 1$}}} and store these vertices along with their colors. Let $S\subseteq V$ be the set of sampled vertices. When a vertex appears in a stream, we check if it forms a monochromatic edge with one of the stored vertices in $S$. At the end of the stream, the algorithm declares the instance of the graph to be properly colored (valid) if it cannot find a monochromatic edge, else it declares the instance to be $\eps$-far from being monochromatic (valid).

We show that Theorem \ref{thm:sep-vardubth} follows easily using Lemma \ref{lem:sunflower}.
\begin{proof} We consider the following two cases.
\begin{itemize}
	\item {Case 1:} There exists a matching of size at least $\sqrt{\vareps m}$: Note that all these matched edges are monochromatic. Let $(u,v)$ denote an arbitrary matched edge where $u$ appears in the stream before $v$. Now, the edge $(u,v)$ will be detected as monochromatic if vertex $u$ has been sampled by the algorithm. The probability that vertex $u$ is sampled is $\frac{10\log n}{\sqrt{m}}$. Since, there are $\sqrt{\vareps m}$ matched monochromatic edges, using Chernoff bounds with probability at least $(1-1/n^2)$, the algorithm will detect at least one of these matched monochromatic edges.

%\[ \begin{aligned}
%\mathcal{P}(\texttt{atleast one of edges of the matching is checked})  \\
%= 1 - \mathcal{P}(\texttt{none of the matching edges are checked}) \\
%= 1 - (1 - p)^{\sqrt{\vareps m}} \geq 1 - e^{-p \sqrt{\vareps m}}
%\end{aligned} \]
%\[ \mathcal{P}(\texttt{a conflicting edge (u, v) is checked}) = \mathcal{P}(\texttt{u is sampled}) = \frac{|S|}{n}  \]
%\[ \begin{aligned}
%\mathcal{P}(\texttt{atleast one of edges of the matching is checked}) = 1 - e^{-p\sqrt{\vareps m}} \\
%= 1 - e^{-\frac{\size{S}}{n}\sqrt{\vareps m}}
%\end{aligned} \]
%So, the sample size is $ \widetilde{\mathcal{O}} \left(\frac{n}{\sqrt{\vareps m}} \right)$. Thus, if we can sample $ \widetilde{\mathcal{O}} \left(\frac{n}{\sqrt{\vareps m}} \right)$ edges, independently with probability $\frac{c\log n}{\sqrt{m}}$, and check them for conflict, we can verify if the coloring function is $\vareps$-far from being valid or not.

	\item {Case 2:} There exists a vertex of degree at least $\sqrt{\vareps m}$: In this case most of the monochromatic edges may be incident on very few high degree vertices. To detect these edges, we want to store either the high degree vertices or one of its neighbours. But, if these high degree vertices appear at the beginning of the stream and we fail to sample them, then we may not detect a monochromatic edge. This is why we assume a \emph{\bf random ordering} of vertices arriving in the stream. Now, assuming random order of vertices in the stream, at least $\frac{1}{5} \sqrt{\vareps m}$ neighbours of $v$ should appear before $v$ in the stream with probability at least $(1-e^{-\frac{9}{50} \sqrt{\vareps m}})$ \remove{\footnote{\comments{If $m$ is small, success probability may be small as well}}}. Since we sample every vertex with probability $\frac{10\log n}{\sqrt{m}}$, with high probability at least $(1-1/n^2)$ one of its neighbours will be stored.

%Since, if the high degree vertex appears at the beginning of the stream and we fail to sample it, then we may not detect a monochromatic edge. A random order stream ensures that the high degree vertex appears after a constant fraction of its neighbors. If we can sample some of the neighbors of the concerned vertex that appear before it in the stream, we can check the conflicting edges. Since the vertices arrive in a random order stream, we claim that the high degree vertex appears after a constant fraction of its neighbors have already been exposed. Let $x$ be the no. of neighbors that appear after the star vertex appears in the random order stream. Then, $\mathbb{E}[x] = \frac{n}{2}$. Let $E$ be the event that the star vertex appears after a constant fraction $(1 - c)$ of its neighbors. Using Markov's inequality, we get, 
%\[ \mathcal{P}(E) = \mathcal{P}(x > cn) \leq \frac{\mathbb{E}[x]}{cn} = \frac{n}{2cn} =  \frac{1}{c'} \] 
%\[
%\begin{aligned}
%\mathcal{P}(\texttt{a conflicting edge is detected}) \geq  \mathcal{P}(E)\mathcal{P}(\texttt{a conflicting edge is detected} |  E) \\
%= \frac{1}{c'} \left(1 - \left(1 - p \right)^{\sqrt{\vareps m}} \right) \geq \frac{1}{c'} \left(1 - e^{-p\sqrt{\vareps m}} \right) \geq \frac{1}{c'} \left(1 - n^{-c} \right)
%\end{aligned}
%\] when the probability of sampling is $p = \frac{c \log n}{\sqrt{m}}$.

%Thus, we are able to check a conflicting edge with high probability.
\end{itemize}
\end{proof}


==> est-lower.tex <==
\section{Lower bounds for \conflictest} \label{sec:est-lowerbound}
 
We show a tight lower bound of $\Omega \left( \min \{ \size{V}, \frac{ \size{E} }{T} \} \right)$ for the \conflictest problem in the vertex arrival model with degree oracle. For the \conflictest problem in the vertex arrival model we show a tight lower bound of $\Omega\left(\min\{\size{V},\frac{|V|^2}{T}\}\right)$. These bounds are proved using reductions from the \emph{INDEX} problem in the one-way communication complexity model to the \conflictest problem in graphs, having atleast $T$ conflicting edges, in the vertex arrival streaming model. In the INDEX problem, Alice gets an $M$-bit string $X\in \{0,1\}^M$ and Bob gets an integer $j\in [M]$. Both Alice and Bob are unaware of each other's input. Alice can send a message to Bob and the goal is for Bob to output $X_j$ with the minimum amount of communication. It is well known that the lower bound on the message length for the INDEX problem in the one-way communication complexity model is $\Omega(M)$ (See Lemma~\ref{index} in Appendix~\ref{sec:comm}).

\subsection{Lower bound for \conflictest in \va model} \label{sec:est-vaaolbsc}

\begin{theorem}\label{theo:est-vaaolbth} Let $n,m,T  \in \N$ be such that $0 \leq T \leq {n \choose 2}$ and $m\geq 2T$. Any one pass streaming algorithm, that takes a coloring function $f:V \rightarrow [C]$ on the vertices\remove{and the edges} of a graph $G(V,E)$ with $\size{V}=\theta(n)$ and $\size{E}=\theta(m)$ in \va model, and determines whether the monochromatic edges in $G$ is $T$ or $2T$ with probability $2/3$, requires 
$\Omega\left( \min \{n,\frac{n^2}{T}\}\right)$ bits of space.
 \end{theorem}

\begin{proof} We show that the lower bound is $\Omega(n)$ when $m > nT$ and $\Omega\left(\frac{n^2}{T}\right)$ when $m \leq nT$, separately, to get the stated lower bound. We give a reduction from the INDEX problem to the \conflictest problem in graphs with $\theta(n)$ vertices, $\theta(m)$ edges and having atleast $T$ conflicting edges, in the vertex arrival model. We show our reduction when $m=2T$, but we can modify it for any $m\geq 2T$.

 The reduction works as follows. For $m > nT$, Alice has a $M$-bit input string $X \in \{0,1\}^{M}$ and an extra bit $X_{M+1}$ is appended. For each input bit $X_i$, Alice creates a vertex $l_i$. If $X_i$ equals $1$, then vertex $l_i$ is colored with color $C_1$, else it is colored with color $C_0$. The vertex $l_{M+1}$ is colored with color $C_1$. After processing all bits of her input, Alice sends the current memory state to Bob. %The space used for the communication is, thus, $\Omega(M+1)$ or $\Omega(M)$. 
Bob constructs a gadget $R$ which is an independent set of $\left(n-M\right)$ vertices and colors all the vertices in the gadget with color $C_{1}$. He adds all the edges from the vertex $l_{j}$ to the gadget $R$. He also adds all the edges from the vertex $l_{M+1}$ to the gadget $R$. The number of vertices is $(M+1) + (n-M) = \Theta(n)$. We set $M=n-T$. If $X_{j} = 0$, then the color of $l_{j}$ is $C_{0}$ and there are $T$ conflicting edges, where as if $X_{j} = 1$, then the color of $l_{j}$ is $C_{1}$ and there will be $2T$ conflicting edges. Therefore, for $M = n-T$, estimating the number of monochromatic edges within a factor of two requires $\Omega(n-T)$ or $\Omega(n)$ space.

For $m \leq nT$, Alice has an $M$-bit input string $X \in \{0,1\}^{M}$ and an extra bit $X_{M+1}$ is appended. For each input bit $X_i$, Alice constructs an independent set $L_{i}$ of size $\frac{2T}{n}$. If $X_i$ equals $1$, then the vertices of $L_{i}$ are colored with color $C_1$, else the vertices are colored with color $C_0$. The vertices of $L_{M+1}$ are colored with color $C_1$. After processing all bits of her input, Alice sends the current memory state to Bob. %The space used for the communication is, thus, $\Omega(M+1)$ or $\Omega(M)$.  
Bob constructs a gadget $R$ which is an independent set of $\frac{n}{2}$ vertices and colors all the vertices with the color $C_{1}$. He adds all the edges from the gadget $L_{j}$ to the gadget $R$. He also adds all the edges from the gadget $L_{M+1}$ to the gadget $R$. We set $M = \frac{n^{2}}{T}$. The number of vertices is $\frac{2T}{n} \cdot( M+1) + \frac{n}{2} = \Theta(n)$.
If $X_{j} = 0$, then the color of vertices in $L_{j}$ is $C_{0}$ and there are $T$ conflicting edges, where as if $X_{j} = 1$, then the color of vertices in $L_{j}$ is $C_{1}$ and there will be $2T$ conflicting edges. Therefore, for $M = \frac{n^{2}}{T}$, estimating the number of monochromatic edges within a factor of two requires $\Omega \left(\frac{n^2}{T} \right)$ space.

Recall that we are doing our reductions for $m=2T$. We make the above constructions work for any $m\geq2T$ by adding a complete subgraph on $\sqrt{m-2T}$ vertices such that none of the edges of the complete subgraph are conflicting.~\footnote{Note that $\sqrt{m-2T}=O(n)$.}
\end{proof} 
 
\subsection{Lower bound for \conflictest in \vadeg model} \label{sec:est-vadglbsc}

\begin{theorem}\label{theo:est-vadglbth} Let $n,T  \in \N$ be such that $0 \leq T \leq {n \choose 2}$. Then there exists an $m$ with $T\leq m \leq {n \choose 2}$ such that the following happens. Any one pass streaming algorithm, that takes a coloring function $f:V \rightarrow [C]$ on the vertices\remove{and the edges} of a graph $G(V,E)$ with $\size{V}=\theta(n)$ and $\size{E}=\theta(m)$ in \vadeg model, and determines whether the monochromatic edges in $G$ is $T$ or $2T$ with probability $2/3$, requires 
$\Omega\left( \min \{n,\frac{m}{T}\}\right)$ bits of space.
 \end{theorem}

\begin{proof} We show that the lower bound is $\Omega(n)$ when $m > nT$ and $\Omega\left(\frac{m}{T}\right)$ when $m \leq nT$, separately, to get the stated lower bound. We give a reduction from the INDEX problem to the \conflictest problem in graphs with $\theta(n)$ vertices, $\theta(m)$ edges and having atleast $T$ conflicting edges, in the vertex arrival model. The existence of $m$ will be evident from the construction.

 The reduction works as follows. For $m > nT$, Alice has a $M$-bit input string $X \in \{0,1\}^{M}$. For each input bit $X_i$, Alice creates a vertex $l_i$. If $X_i$ equals $1$, then vertex $l_i$ is colored with color $C_{i1}$, else it is colored with color $C_{i0}$.  After processing all bits of her input, Alice sends the current memory state to Bob. %The space used for the communication is, thus, $\Omega(M+1)$ or $\Omega(M)$. 
 Let $j \in [M]$ be the input of Bob. Bob constructs a gadget $R\cup\{b\}$ of $n-M+1$ vertices such that $R$ is an independent set of $\left(n-M\right)$ vertices and $b$ is a singleton vertex. Bob colors all the vertices in the gadget $R\cup \{b\}$ with color $C_{j1}$. He adds all the edges from $R$ to all the vertices in $\{l_i:i \in [M]\}\cup \{b\}$. The number of vertices is $M+ (n-M)+1 = \Theta(n)$. We set $M=n-T$. If $X_{j} = 0$, then the color of $l_{j}$ is $C_{j0}$ and there are $T$ many conflicting edges between $b$ and the vertices in $R$, where as if $X_{j} = 1$, then the color of $l_{j}$ is $C_{j1}$ and there will be $2T$ many conflicting edges. Therefore, for $M = n-T$, estimating the number of monochromatic edges within a factor of two requires $\Omega(n-T)$ or $\Omega(n)$ space.

For $m \leq nT$, Alice has an $M$-bit input string $X \in \{0,1\}^{M}$. For each input bit $X_i$, Alice constructs an independent set $L_{i}$ of size $\frac{2nT}{m}$. If $X_i$ equals $1$, then the vertices of $L_{i}$ are colored with color $C_{i1}$, else the vertices are colored with color $C_{i0}$. After processing all bits of her input, Alice sends the current memory state to Bob. %The space used for the communication is, thus, $\Omega(M+1)$ or $\Omega(M)$.  
Let $j \in [M]$ be the input of Bob. Bob constructs a gadget $R\cup {B}$ where $R$ is an independent set of $\frac{m}{2n}$ vertices and $B$ is an independent set of $\frac{2nT}{m}$ vertices. Bob colors the vertices in $R\cup B$ with $C_{j1}$ and he adds all the edges from $R$ to 
$B \cup L_i$, for all $i \in [M]$. We set $M = \frac{m}{T}$. The number of vertices is $\frac{2nT}{m} \cdot M + \frac{m}{2n}+\frac{2nT}{m} =\theta(n)$ as $T \geq \frac{n}{2}$ and $m \geq T$.
If $X_{j} = 0$, then the color of vertices in $L_{j}$ is $C_{j0}$ and there are $T$ conflicting edges, where as if $X_{j} = 1$, then the color of vertices in $L_{j}$ is $C_{j1}$ and there will be $2T$ conflicting edges. Therefore, for $M = \frac{m}{T}$, estimating the number of monochromatic edges within a factor of two requires $\Omega \left(\frac{m}{T} \right)$ space.
\end{proof}


\remove{
Comments:
\begin{enumerate}
	\remove{\item \comments{Total number of vertices is more than $n$. I guess asymptotically we are fine, still would be good to mention.}}
	\item \comments{Number of vertices in $R$ is $\frac{MT}{n}=\frac{m}{n}$, which may be less than $1$ for $m<n$}
	\item \comments{How do we show that the degree queries do not help?}
\end{enumerate}
}

















==> graph_algortihms.tex <==
\section{General Problems--Separation of \iporacle{} query and {\sc Local} query}
In this section we discuss deciding connectivity and finding edges in a global minimum cut to show that when given access to inner product oracle of the adjacency matrix of the graph.

Let $G = (V,E)$, $|V| = [n]$ and let $A$ be the corresponding adjacency matrix of $G$ whose rows and columns are indexed by $V$. Without loss of generality assume $n$ to be power of $2$. For a vertex $i \in V$, let $N_i(G) \subseteq V$ denote the set of neighbours of $i$ in $G$. We begin with the observation that given inner product access to $A$, for any $i \in V$ and $S \subseteq V$, the set $N_i(G) \cap S$ can be found deterministically  using at most $O(|N_i(G) \cap S| \log n)$ many \iporacle{} queries.

\remove{\paragraph{Algorithm: {\sc{Find-First-Restricted-Neighbour}}($i, S$)}
\begin{itemize}
    \item \textbf{Input:} \iporacle{} access to the adjacency matrix $A$ of $G = (V,E)$, a vertex $i \in V$ and $S \subseteq V$
    
    \item \textbf{Output:} $k = \min\{N_i(G) \cap S\}$ if $|N_i(G) \cap S| \neq 0$, $0$ otherwise.
    
    \item \textbf{Initialization:} $\boldvec{x} = \boldvec{1_S}$
    
    \item If $\dpd{A_{i,*}}{\boldvec{1}} = 0$, return $0$
    
    \item repeat:
    \begin{itemize}
        \item Form a vector ${\bf{y}}$ (${\bf{z}}$) in $\{0,1\}^n$ by setting second (first) half of the nonzero elements in $\boldvec{x}$ to $0$ and keeping the remaining elements unchanged.
        
        \item Determine $\ell = \dpd{A_{i,*}}{\bf{y}}$ and $r = \dpd{A_{i,*}}{\bf{z}}$.
        
        \item If $\ell = 1$ and number of $1$'s in $\boldvec{x} = q$, then return the non-zero coordinate of $\boldvec{x}$.
    
        \item If $\ell = 0$ set $\boldvec{x} = \boldvec{z}$
        \begin{itemize}
            \item Else set $\boldvec{x} = \boldvec{y}$
        \end{itemize}
    \end{itemize}
\end{itemize}
}

\begin{obs}
\label{lem:graph_first_neigh}
 Let $G(V,E)$ be a graph. Given a vertex $v \in V(G)$ and $S \subseteq V(G)$ as input, all the neighbors of $v$ in $S$, that is, $N_G(v) \cap S$ can be determined by using $\Oh({|N_G(v) \cap S|\log |S|}+1)$ {\sc Induced Degree} queries to graph $G$.
\end{obs}
\begin{proof}
We first $|N_G(v) \cap S|\neq 0$ as this can be decided by using just one {\sc Induced Degree} query. Now we describe the algorithm in a recursive manner. Observe that, as we have access to {\sc Induced Degree} query, we can report a neighbor of $v$ in $S$ by using $\log |S|$ many queries by using binary search. Let $u$ be the neighbor that is reported first by tha lgorithm by using $\log |S|$ many queries. Now, we recurse to find the neighbors of $v$ in $S \setminus \{u\}$ in the similar fashion.  So, the total number of queries made by the algorithm is $\Oh({|N_G(v) \cap S|\log |S|}+1)$.
%We first check whether $N_G(v) \cap S =\emptyset$. If yes, we return the same and quit. Otherwise, we partition $S$ into two roughly equal parts $S_1$ and $S_2$. Find $N_G(v) \cap S_1$ and $N_G(v) \cap S_1$ recursively and report the union. We prove the query complexity, of our algorithm, is ${|N_G(v) \cap S|\log n}$ by using induction on $|N_G(v) \cap S|$. Note that the base case, when ${|N_G(v) \cap S|}=0$ , trivially holds as we can report it by using only one query. For the inductive step, the number of queries made by the algorithm is bounded by ${|N_G(v) \cap S_1|\log n}+{|N_G(v) \cap S_2|\log n}=|N_G(v) \cap S|\log n}$.

\end{proof}

\paragraph{Algorithm: {\sc{Find-Restricted-Neighbourhood}}($i, S$)}
\begin{itemize}
    \item \textbf{Input:} \iporacle{} access to the adjacency matrix $A$ of $G = (V,E)$, a vertex $i \in V$ and $S \subseteq V$
    
    \item \textbf{Output:} $N_i(G) \cap S$.
    
    \item \textbf{Initialization:} $N = \phi$ and $T = S$.
    
    \item while {\sc{Find-First-Restricted-Neighbour}}($i, T$) $\neq 0$:
    \begin{itemize}
        \item $N = N \cup~${\sc{Find-First-Restricted-Neighbour}}($i, T$)
        
        \item $T = T \setminus~${\sc{Find-First-Restricted-Neighbour}}($i, T$)
    \end{itemize}
    
    \item return $N$
\end{itemize}


\begin{obs}
\label{lem:graph_neighbourhood_vertex}
{\sc{Find-Restricted-Neighbourhood}} takes $i \in [n]$ and $S \subseteq [n]$ as input, outputs the set of $N_i(G) \cap S$ by using $\Oh(|N_i(G) \cap S| \log n)$ \iporacle{} many queries to matrix $A$.
\end{obs}

\paragraph{Algorithm: {\sc{Breadth-First-Search}}}
\begin{itemize}
    \item \textbf{Input:} \iporacle{} access to the adjacency matrix $A$ of $G = (V,E)$.
    
    \item \textbf{Output:} The set of connected components of $G$.
    
    \item \textbf{Initialization:} Let $Q = \phi$ be the queue data structure. Let $B$ be an array of length $n$ initialized with $0$ i.e. $B[i] = 0$ for all $i \in [n]$.
    
    \item For $i \in [n]$:
    
    If $B[i] = 0$ then $Q = Q \cup i$:
    
    While $Q \neq \phi$:
    
    let $i \leftarrow Q$
    
    if {\sc{Find-Restricted-Neighbourhood}}($i, V$)$~\neq \phi$:
    \begin{itemize}
        \item for $j \in~${\sc{Find-Restricted-Neighbourhood}}($i, V$) such that $B[j] = 0$:
        \begin{itemize}
            \item $B[j] = i$
            \item $Q = Q \cup j$
        \end{itemize}
    \end{itemize}

    \item Return $B$
\end{itemize}

\textcolor{blue}{Manaswi: proof of lower bound of $\Omega(n)$, to write: the statement. The lower bound is for randomized \iporacle{} query algorithm also}

\begin{proof}
    For lower bound, consider the following version of unique set intersection promised in communication complexity: Alice is give $x \in \{0,1\}^n$ and Bob is given $y \in \{0,1\}^n$. The players want to output $1$ if there is an $i \in [n]$ such that $x_i = y_{i+1} = 1$, where the indices of $x$ and $y$ are modulo $n$. Furthermore, it is promised that either there is a unique $i \in [n-1]$  such that $x_i = y_{i+1} = 1$ or there is no such $i$.
    
    For reduction construct the matrix $A \in \{0,1\}^{n \times n}$ as follows: if $x_i = y_{i+1} = 0$ then $A(i,i+1) = 1$, $1$ otherwise, where the indices of $x$ and $y$ are modulo $n$. Note that under the promise of the communication problem the graph corresponding to $A$ is a line graph on $n$ vertices if and only if $x$ and $y$ do not intersect. Otherwise the corresponding graph is a disconnected graph. 
    
    Now Alice and Bob simulate the query algorithm for connectivity to solve the disjointness problem. Since each row of $A$ contains at most a single $1$, every \iporacle{} query can be simulated using a single bit. This gives the desired $\Omega(n)$ lower bound.
\end{proof}


\subsection{Separation of \iporacle{} query and {\sc Local} query through Global Minimum Cut:}
\color{blue}
First we discuss that \iporacle{\{0,1\}^n} as an unified framework for local queries along with such as {\sc Degree}, {\sc Adjacency} and {\sc Neighbor} query. Let us consider the adjacency matrix $A$ of an unweighted and undirected graph $G$. Let $V(G)=[n]$. The degree of a vertex $a \in [n]$ is $\dpd{A_{a*}}{\vecone}$ and $(a,b) \in E(G)$ if and only if $\dpd{A_{a*}}{{\bf{v}}}=1$, where ${\bf{v}}$  is the vector such that $v_b=1$ and $v_k =0$ for $k \neq b$. So, degree and adjacency queries  are special cases of \iporacle{\{0,1\}^n} query. Also, observe that the $i$-th neighbor of a given vertex $a$ can be determined by $\log n$ many \iporacle{\{0,1\}^n} queries. Hence, \iporacle{\{0,1\}^n} has an unified framework for all local queries in a graph.
The proposed inner product query oracle encompasses the local queries. Note that inner product query is also a type of local query in case of matrices.

As \iporacle{} query is \emph{stronger} than {\sc Local} query, it is a natural question to ask ``Does there exists a natural problem where \iporacle{} query outperforms {\sc Local} query''? We answer this question in the positive direction through Global Minimum Cut.
\color{black}
--\complain{This might move to intro.}

 The following proposition says that we need to make $\Omega(m)$ local queries to find all the edges of a global minimum cut of an unknown graph using local queries. however, this problem of finding all the edges of a global minimum cut can be bound by using $\widetilde{\Oh}\left(\frac{m}{t}\right)$ many \iporacle{} queries (See Theorem~\ref{theo:cutfind}).
\begin{pre}\label{pro:lb-mincut-findings}~\cite{DBLP:journals/corr/abs-2007-09202}
   Let $m,n,t \in \N$ with $t \leq n-1$ and $ 2nt \leq m \leq {n \choose 2}$. Any algorithm, that finds all the edges in a minimum cut of an unknown graph $G$ with $\size{V(G)} = n$, $\size{E(G)} = m$ and $\size{\mbox{\sc Cut}(G)} = t$ with probability $2/3$, must make at least $\Omega(m)$ queries in order to find. Here each query is one out of {\sc Degree}, {\sc Neighbor}, {\sc Adjacency} or {\sc Random Edge} query.
\end{pre}
Bishnu et al.~\cite{DBLP:journals/corr/abs-2007-09202} shown that 
the size of the minimum cut can be estimated by using $\widetilde{\mathcal{O}}\left(\frac{m}{t}\right)$ many {\sc Local} queries. This imples we can also estimate the size of the minimum cut by using $\widetilde{\mathcal{O}}\left(\frac{m}{t}\right)$ many \iporacle{} queries. 
\begin{pre}\label{pro:cut-est}
    There exists an algorithm that given a {\sc Local}/\iporacle{} query access to a unknown graph $G$ and $\eps \in (0,1)$ as inputs, give an $(1\pm \eps)$-approximation to $\size{\mbox{\sc Cut}(G)}$, i.e., the size of the minimum cut of $G$ with high probability. Moreover, the algorithm uses $\widetilde{\mathcal{O}}\left(\frac{m}{t}\right)$ 
many queries, where $m= \size{E(G)}$ and $t = \size{\mbox{\sc Cut}(G)}$.
Note that $\widetilde{\mathcal{O}}\left( \cdot \right)$ hides polynomial terms in $\log n$ and $\frac{1}{\epsilon}$ where $n = \size{V(G)}$.
\end{pre}
\begin{theo}\label{theo:cutfind}[Separating local and \iporacle{} queries]
 \comments{Algorithm~\ref{algo-exact-min-cut} computes the minimum cut using $\widetilde{\mathcal{O}}\left( \frac{m}{t}\right)$, where $m = \size{E}$ and $t = \mbox{{\sc Cut}}_{2} \left( G\right)$, with probability at least $1-\frac{1}{n^{10}}$.}
    \label{thm:induced-degree-mincuts}
\end{theo}
\begin{proof}
    We will first prove the correctness of the algorithm.
    Observe that from Lemma~\ref{lem:karger}, with probability at least $1 - \frac{1}{n^{10}}$, all cuts $\mbox{Cut}^{2}_{G}(A_{1}, A_{2})$ satisfy the following inequality:
    $$
        (1-\eps)p \leq
        \frac{\size{\mbox{{\sc Cut}}^{2}_{\widetilde{G}}(A_{1}, A_{2})}}{\size{\mbox{{\sc Cut}}^{2}_{{G}}(A_{1}, A_{2})}}
        \leq (1+\eps)p.
    $$
    Also, note that this implies that if $\size{\mbox{{\sc Cut}}^{2}_{\widetilde{G}} (A_{1}, A_{2})} \leq (1+\eps)p\hat{t}$, then $\size{\mbox{{\sc Cut}}^{2}_{\widetilde{G}} (A_{1}, A_{2})} \leq (1+4\eps) p \mbox{{\sc Cut}}_{2}(G)$. Note that, from Theorem~\ref{prop-KawarabayashiT15}, this implies that ``Failure'' case in {\bf Step 4} of Algorithm~\ref{algorithm-finding-mincut} does not happen with probability at least $1 - \frac{1}{n^{10}}$.
    Therefore Algorithm~\ref{algorithm-finding-mincut} computes the exact minimum cut with probability at least $1-\frac{1}{n^{10}}$.
    
    Observe that using $O\left( \log n\right)$ many \iporacle{} queries we can simulate the $j$-neighbor query of a vertex. Using Lemma~\ref{algorithm-finding-mincut} together with this observation, we can implement {\bf Step 1} of Algorithm~\ref{algorithm-finding-mincut} using $\widetilde{\mathcal{O}}\left( \frac{m}{t}\right)$ many \iporacle{} queries. For {\bf Step 2} and {\bf Step 3} of the Algorithm~\ref{algorithm-finding-mincut} we are not using any \iporacle{} queries. For {\bf Step 4} of the Algorithm~\ref{algorithm-finding-mincut}, observe that, using Lemma~\ref{lem-finding-all-neighbors-induced-degree} and the fact that $n \leq \frac{m}{t}$, we will be using using $\widetilde{\mathcal{O}}\left( n\right) = \widetilde{\mathcal{O}}\left( \frac{m}{t} \right)$ many \iporacle{} queries. Putting together everything, the total number of induced queries used by our algorithm will be bounded by $\widetilde{\mathcal{O}}\left( \frac{m}{t}\right)$.
\end{proof}
\begin{theo}
    There exists an algorithm that given a  \iporacle{} query access to a unknown graph $G$ and $\eps \in (0,1)$ as inputs can the $\size{\mbox{\sc Cut}(G)}$, i.e., the size of the minimum cut of $G$ with high probability. Moreover, the algorithm uses $\widetilde{\mathcal{O}}\left(\frac{m}{t}\right)$ 
many queries, where $m= \size{E(G)}$ and $t = \size{\mbox{\sc Cut}(G)}$.

Note that $\widetilde{\mathcal{O}}\left( \cdot \right)$ hides polynomial terms in $\log n$ and $\frac{1}{\epsilon}$ where $n = \size{V(G)}$.
\end{theo}

Now we will show that using \iporacle{} query, we can find exact minimum cut efficiently. 

We will assume that $0< \eps \leq 1/5$, and we have an estimate $\hat{t}$ of the minimum cut value $\size{\mbox{{\sc Cut}}_{2}(G)}$ satisfying the following:
$$
    \frac{1}{1+\eps}\leq \frac{\hat{t}}{\size{\mbox{{\sc Cut}}_{2}(G)}} \leq 1+\eps
$$
\begin{lem}
\label{lem-finding-all-neighbors-induced-degree}
    Note that we can find such an estimate for $\size{\mbox{{\sc Cut}}_{2}(G)}$ using the algorithms in the previous section using $\widetilde{\mathcal{O}}\left( \frac{m}{t}\right)$ many local queries where $t = \size{\mbox{{\sc Cut}}_{2}(G)}$.  \textcolor{blue}{cite some suitable paper, like one we submitted to SODA.}    
\end{lem}


The following theorem shows the hardness of finding the minimum cut using local and random edge queries. \textcolor{blue}{this line is not needed.}


Without loss of generality, assume that the minimum cut is not a singleton cut in the graph. 


\begin{algorithm}
\SetAlgoLined
\caption{{\sc Finding exact minimum cut}($\eps$)}
\label{algo-exact-min-cut}
\KwIn{\iporacle{} access to the graph $G$.}
\KwOut{Exact minimum cut $\mbox{{\sc Cut}}_{2}(G)$ of $G$.}
\begin{description}
    \item[Step 1.]
        Sample each edge of $G$ with probability $p = \min\left\{ \frac{200(1+\eps)\log n}{\eps^{2} \hat{t}}, \, 1\right\}$ to obtain the subgraph $\widetilde{G}= (V, E_{p})$ of $G$.
    
    
    \item[Step 2.]
        Compute all non-singleton cuts in $\widetilde{G}$ of size at most $(1+\eps)p\hat{t}$. 
        
    \item[Step 3.]
    We will now construct a partition of the vertex set $V$ using the cuts computed in {\bf Step 2}.
    Contract any two
        vertex belongs to the same partition if they are together in all such cuts computed in {\bf Step 2}. 
    Without loss of generality, let the partition of $V$ be $V = \cup_{i=1}^{t} V_{i}$ for some $t \in [n]$. 
    \item[Step 4.]
        We will now construct a new multigraph $\widehat{G}$ whose vertex set is $\{V_{1}, \, \dots, \, V_{t}\}$ and the edges corresponds to the edges in $G$ going across all $V_{i}$ and $V_{j}$ where $i, \, j \, (i\neq j) \in [t]$. We learn all the edges in $\widehat{G}$ using \iporacle{} queries, unless the number of edges in $\widehat{G}$ becomes more than $n\log n$, in which case we report a ``Failure'' and terminate the algorithm. 
        
    \item[Step 5.] Output the minimum cut in the graph $\widehat{G}$.
\end{description}
\label{algorithm-finding-mincut}
\end{algorithm}

We will now prove the following theorem. 




To completely the proof of Theorem~\ref{thm:induced-degree-mincuts} we will need the following two results. 

\begin{theo}[Kawarabayashi and Thorup~\cite{KT15deterministic}]
    Let $G = (V(G), E(G))$ with minimum degree $d$ and minimum cut value $c$. For $\eps \in [0,1)$, let $\mathcal{C}(\eps)$ be the family of all non-singleton cuts in the graph in $G$ with cut value at most $c + \eps d$. Then number of edges of $G$ that is participating in at least one of the cuts from $\mathcal{C}({\eps})$ is bounded by $O(n)$.
    \label{prop-KawarabayashiT15}
\end{theo}

\begin{lem}\label{lem-finding-all-neighbors-induced-degree}
        Let us assume that the query algorithms have access to \iporacle{} query to an unknown graph $G = (V(G), E(G))$. 
        There exists an algorithm that takes as input a subset $S$ of $V(G)$ and $v \in V(G)$, and outputs the set $S\cap N(v)$ using $\mathcal{O}\left(\size{S\cap N(v)}+\size{S\cap N(v)}\log n\right)$ many queries, where $n = \size{V(G)}$.
\end{lem}
\begin{proof}
    Observe that just using binary search we can find one element of $u \in S\cap N(v)$ using $\mathcal{O}\left( 1 + \log n\right)$ many \iporacle{} queries. We then use recursion on the set $S\setminus \{u\}$ to find the rest of neighbors of $v$ in the set $S$. Total number of \iporacle{} queries used will be $\mathcal{O}\left(\size{S\cap N(v)}+\size{S\cap N(v)}\log n\right)$. \textcolor{blue}{Manaswi: another binary search algo in General graph section}
\end{proof}


\subsection{Some query models}
Definition of some queries that might be useful later:
\begin{itemize}
    \item 
        {\sc Demand} query: A Demand Query takes as input a vertex $i \in V(G)$ and an order on a subset of vertices $(i_{1}, \, \dots, i_{k})$, where $i_{j} \in V(G) \setminus \{i\}$, and the query reports the first vertex $i_{j}$ in such that $\{i, i_{j}\} \in E(G)$ in the graph, otherwise outputs a special symbol $\perp$ to denote that none exists, i.e., if 
        the query outputs $i_{j}$ then for all $\ell < i$,
        we have $\{i, i_{\ell}\} \not\in E(G)$.
        
        \item 
        $\mbox{{\sc Approx-degree}}_{\alpha}$ query: The query takes as input $i \in V(G)$, and outputs $\hat{d}_{i}$ where $\hat{d}_{i}$ is an $(1\pm \alpha)$-approximation of the degree $d_{i}$ of $i$ in $G$.
        
        \item
        {\sc Random-neighbor} query: The query takes as input $i \in V(G)$ and outputs a random neighbor of $i$ in $G$.
\end{itemize}

Using {\sc Demand} query we can efficiently simulate both $\mbox{{\sc Approx-degree}}_{\delta}$ query and {\sc Random-neighbor} query.

\begin{lem}\label{lem-implement-with-demand}
    Let $G$ be a unknown graph with vertex set $V(G) = [n]$, and we have {\sc Demand} query access to $G$. Then
    \begin{itemize}
        \item[(i)]
            {\sc Random-neighbor} query can be implemented using one {\sc Demand} query.
        
        \item[(ii)]
            $\mbox{{\sc Approx-degree}}_{\alpha}$ query can be implemented, with probability at least $1-\frac{1}{n^{10}}$, using $\mathcal{O}\left( \frac{\log n}{\alpha^{2}}\right)$ many {\sc Demand} queries.
    \end{itemize}
\end{lem}
\begin{proof}
    \begin{itemize}
        \item[(i)] 
            Let $i$ be the vertex whose random neighbor we want to find. If we call {\sc Demand} query with the vertex $i$ and a uniformly random ordering of the set $[n]\setminus\{i\}$ then we will get a uniformly random neighbor of $i$ in $G$.  
            
        \item[(ii)]
            The result is a direct consequence of \cite[Lemma~2.9]{DBLP:journals/corr/abs-1711-07567}. 
    \end{itemize}
\end{proof}

We will first prove the following result. 

\begin{theo}
    There exists an algorithm that given a  {\sc Random-neighbor} query and $\mbox{{\sc Approx-degree}}_{\eps/16}$ query access to a unknown graph $G$ and $\eps \in (0,1)$ as inputs can compute a $(1 \pm \eps)$-approximation to $\size{\mbox{\sc Cut}(G)}$, i.e., the size of the minimum cut of $G$ with high probability. Moreover, the algorithm uses $\widetilde{\mathcal{O}}\left(\frac{m}{t}\right)$ 
many queries, where $m= \size{E(G)}$ and $t = \size{\mbox{\sc Cut}(G)}$.

Note that $\widetilde{\mathcal{O}}\left( \cdot \right)$ hides polynomial terms in $\log n$ and $\frac{1}{\epsilon}$ where $n = \size{V(G)}$.
\end{theo}

Using Lemma~\ref{lem-implement-with-demand} with the above theorem, we get

\begin{theo}
    There exists an algorithm that given a  {\sc Demand} query access to a unknown graph $G$ and $\eps \in (0,1)$ as inputs can compute a $(1 \pm \eps)$-approximation to $\size{\mbox{\sc Cut}(G)}$, i.e., the size of the minimum cut of $G$ with high probability. Moreover, the algorithm uses $\widetilde{\mathcal{O}}\left(\frac{m}{t}\right)$ 
many queries, where $m= \size{E(G)}$ and $t = \size{\mbox{\sc Cut}(G)}$.

Note that $\widetilde{\mathcal{O}}\left( \cdot \right)$ hides polynomial terms in $\log n$ and $\frac{1}{\epsilon}$ where $n = \size{V(G)}$.
\end{theo}
\remove{
\subsection{Lemmas taken from SODA paper}
\begin{lem}[Karger~\cite{Karger93}]
\label{lem:karger_cut_bound}
For a given graph $G$ the number of cuts in $G$ of size at most $j \cdot \size{\mbox{\sc Cut}(G)}$ is at most $n^{2j}$.
\end{lem}

\begin{lem}
\label{lem:karger}
Let $G$ be a graph, $ \hat{t} \leq t = \size{\mbox{\sc Cut}(G)}$ and $\eps \in (0,1)$. If $H(V(G), E_p)$ be a subgraph of $G$ where each edge in $E(G)$ is included in $E_p$ with probability $p = \min \left\{\frac{200 \log n}{\eps^2 \hat{t}},1 \right\}$ independently, then every cut of size $k$ in $G$ has size $pk(1 \pm \eps)$ in $H$ with probability at least $1-\frac{1}{n^{10}}$.
\end{lem}

\begin{proof}[Proof of Lemma~\ref{lem:karger}]
If $p=1$, we are done as the graph $H$ is exactly same as that of $G$. So, without loss of generality assume that the graph $G$ is connected. Otherwise, the lemma holds trivially as $\size{\mbox{\sc Cut}(G)} =0$, i.e., $\hat{t}=0$ and $p=1$. Hence, for the rest of the proof we will assume that $p=\frac{200\log n}{\eps^2 \hat{t}}$.

%If a $r$-cut of size $k$ in $G$ has size $pk(1 \pm \eps)$ in $H$, then we say
%the $r$-cut is approximately preserved in $H$. 
Consider a cut $\cC_G(A_{1}, A_{2})$ of size $k$ in $G$. As we are sampling each edge with probability $p$, the expected size of the cut $\cC_H(A_{1}, A_{2})$ is $pk$. Using Chernoff bound (see Lemma~\ref{lem:chernoff} in Section~\ref{sec:prob}), we get
\begin{equation}\label{eq:cher}
     \pr \left(\size{\mbox{$\cC_H(A_{1},A_{2})-pk$}} \geq \eps pk  \right) \leq e^{-\eps^2pk/3\hat{t}} 
             = n^{-\frac{100k}{3\hat{t}}}
\end{equation}

Note that here we want to show that every cut in $G$ is approximately preserved in $H$. To do so, we will use Lemma~\ref{lem:karger_cut_bound} along with Equation~\ref{eq:cher} as follows.  
Let $Z_1,Z_2,\ldots,Z_{\ell}$ be the partition of the set of all cuts in $G$ such that each cut in $Z_j$ has the number of edges between $\left[j\cdot \size{\mbox{\sc Cut}(G)},(j+1)\size{\mbox{\sc Cut}(G)}\right]$, where $\ell \leq \frac{n}{\size{\mbox{\sc Cut}(G)}}$ and $j \leq \ell-1$. From Lemma~\ref{lem:karger_cut_bound}, $\size{Z_j} \leq n^{2j}$. Consider a particular $Z_j, j \in [\ell]$. Using the union bound along with Equation~\ref{eq:cher}, the probability that there exists a cut in $Z_j$ that is not approximately preserved in $H$ is at most $\frac{1}{n^{11}}$. Taking union bound over all $Z_j$'s, the probability that there exists a cut in $G$ that is not approximately preserved is at most $\frac{1}{n^{10}}$.
\end{proof}}

==> macro-this-paper.tex <==
\newcommand{\ealong}{{\sc Edge Arrival}\xspace}
\newcommand{\ea}{{\sc EA}\xspace}
\newcommand{\dealong}{{\sc Dynamic Edge Arrival}\xspace}
\newcommand{\dea}{{\sc DEA}\xspace}
\newcommand{\valong}{{\sc Vertex Arrival}\xspace}
\newcommand{\va}{{\sc VA}\xspace}
\newcommand{\vadeglong}{{\sc Vertex Arrival with Degree Oracle}\xspace}
\newcommand{\vadeg}{{\sc VAdeg}\xspace}
\newcommand{\varandlong}{{\sc Vertex Arrival in Random Order}\xspace}
\newcommand{\varand}{{\sc VArand}\xspace}
\newcommand{\allong}{{\sc Adjacency List}\xspace}
\newcommand{\al}{{\sc AL}\xspace}
\newcommand{\colorverify}{{\sc Conflict-Sep}\xspace}
\newcommand{\conflictest}{{\sc Conflict-Est}\xspace}
\newcommand{\listcolor}{{\sc List-Coloring}\xspace}
\newcommand{\approxlistcolor}{{\sc Approx-List-Coloring}\xspace}

\newcommand{\strmlistgraph}{{\sc Graph-Strm-List-Coloring}\xspace}
\newcommand{\strmlisthyper}{{\sc Hypergraph-Strm-List-Coloring}\xspace}
\renewcommand{\somecommand}{\begin{something}\somecommand\end{something}}

\renewcommand{\hat}{\widehat}
\renewcommand{\tilde}{\widetilde}
\renewcommand{\Tilde}{\widetilde}

==> other-upper.tex <==
\remove{
\section{\conflictest in \va model}\label{sec:est-vaaoubsc}

When $T< n/2$, we show that there are no space efficient streaming algorithms for \conflictest. That is any streaming algorithm requires to store all $n$ vertices along with their colors. It is immediate that in this case one can exactly count the number of monochromatic edges, $\size{E_M}$, in the graph. 
%To estimate the number of monochromatic edges in the arbitrary order \va model when $T < \frac{n}{2}$, we store all the vertices and their colors. When a vertex $v$ arrives in the stream, we store $v$ and its color and all edges of the form $(u,v)$ are checked for conflict, where $u$ is a neighbor of $v$ that appears to its left in the stream. Since all the vertices and their colors are stored, we are able to check each edge for conflict and give an accurate count of the number of monochromatic edges.

When $T \geq \frac{n}{2}$, we sample a subset of $\widetilde{\mathcal{O}}\left(\frac{n^{2}}{T}\right)$ vertex pairs and their colors. The algorithm in this case is an extension of the algorithm in the vertex arrival model with degree oracle given in Sec.~\ref{sec:est-vaubsc}. Here, for a sampled vertex, we store it along with its color and also store its $j^{th}$ neighbor appearing to its right in the stream, where $j \in [n-1]$. However, this neighbor may or may not exist. If it does, we check the corresponding edge for conflict. The number of edges we effectively sample is $\widetilde{\mathcal{O}}\left(\frac{n^{2}}{T}\right)$, independently and uniformly at random with probability $\widetilde{\mathcal{O}}\left(\frac{1}{T}\right)$ each. We check each of the sampled edges for conflict and using this count, estimate the total number of monochromatic edges in the graph.

\remove{When a vertex $u$ arrives in the stream, we store $u$ and its color, if it is sampled. We store the $j^{th}$ neighbor of $u$ appearing to its right in the stream, where $j \in [n-1]$. If the $j^{th}$ neighbor of $u$ exists, we check the corresponding edge for conflict. The number of edges effectively sampled is $\widetilde{\mathcal{O}}\left(\frac{n^{2}}{T}\right)$, independently and uniformly at random with probability $\widetilde{\mathcal{O}}\left(\frac{1}{T}\right)$ each. We check each of the sampled edges for conflict and using this count, estimate the total number of monochromatic edges in the graph.}

%\comments{Anup: Confusing. Checking for $j$th neighbour on the right is not easy in vertex arrival model. Also, it is not clear whether we are sampling vertices or edges. I think it may be possible to rewrite it such that all $n^2/T$ pairs are generated before the stream starts. During the stream we store colors of vertices for these pairs and during or at the end of the stream, check how many of these pairs are monochromatic.}

 \begin{theorem} \label{theo:est-vaaoubth}
 Given any input graph $G = (V, E)$ and a coloring function $f : V(G) \rightarrow [C]$, we can solve the \conflictest problem in the arbitrary order \va streaming model with high probability in 
 $ \widetilde{\mathcal{O}} \left( \min \left( \size{V},\frac{|V|^2}{T} \right) \right) $ space, where $T$ is a lower bound on the number of monochromatic edges in the graph.
 \end{theorem}

\begin{proof}

When $T < \frac{n}{2}$, we store all the vertices and their colors. So, the space required to compute the number of monochromatic edges is $\Omega(n)$.
When $T \geq \frac{n}{2}$, we sample a vertex $u$ and its color $f(u)$ in the stream.
\[
 \mathcal{P}\left(\texttt{an edge e is conflicting}\right) \geq \frac{T}{ {n \choose 2}} \geq \frac{T}{n^{2}}
 \]
If we sample $t$ edges overall, independently and uniformly at random, then,
\[
 \mathcal{P}(\texttt{none of the edges sampled are conflicting}) \leq \left(1-\frac{T}{n^{2}} \right)^t \leq e^{-\frac{Tt}{n^{2}}}
\]
Effectively, we sample and check $\widetilde{\mathcal{O}}\left(\frac{n^{2}}{T} \right)$ edges for conflict. 
Let $S$ be the number of monochromatic edges in the sample of edges selected and let $C$ be the total number of monochromatic edges in the graph. We assume an ordering of the monochromatic edges in the graph. To estimate the number of monochromatic edges in the graph, we do the following:
Let $S_{i}$ be an indicator random variable defined as follows:
 \[  S_{i} = \left\{
        \begin{array}{ll}
            1 & \quad \text{if the } i^{th} \text{ monochromatic edge is sampled with probability } \widetilde{\mathcal{O}}\left(\frac{1}{T}\right) \\
            0 & \quad \text{otherwise}
        \end{array}
    \right.
\] 
 $S = \sum S_{i}$
 \[  \mathbb{E} [S] = \mathbb{E} \left[ \sum S_{i} \right] = \sum \mathbb{E} \left[S_{i} \right] = \sum \frac{k \log n}{T} = \frac{k C \log n}{T}  \]
for some constant $k$.
Thus, the expected number of monochromatic edges in the sample is $\mathbb{E} [S]= \frac{k C \log n}{T} $.  The algorithm calculates the sample size $S$ and reports the number of monochromatic edges in the graph as $C^{'}$, where $C^{'} = \frac{k^{'} S T}{\log n}$ for some constant $k^{'}$ and $\mathbb{E} [C^{'}] = C$.
 \[  \mathcal{P} \left(\size{C' - C} \geq \vareps C \right) = \mathcal{P} \left(\size{S - \frac{10C \log n}{\vareps^{2}T}} \geq \frac{10 C \log n}{\vareps T} \right)   \]
 Applying Chernoff bound (See Lemma~\ref{lem:cher_bound1} in Appendix~\ref{sec:prob}), we get:
 \[  \mathcal{P}\left(\size{S - \frac{10C \log n}{\vareps^{2}T}} \geq \frac{10 C \log n}{\vareps T} \right) \leq 2 \exp \left(-\frac{10 C \log n}{\vareps^{2}T}\frac{\vareps^{2}}{3} \right) \leq 2n^{-3}   \]
 since $C > T$.
 With high probability, we can solve the \conflictest problem in $\widetilde{\mathcal{O}}\left(\frac{n^{2}}{T} \right)$ space in the vertex arrival model when $T \geq \frac{n}{2}$.
\end{proof} 
}

\subsection{\colorverify in \vadeg model} \label{sec:sep-vadegubsc}

In this variant, we solve the \colorverify problem for graphs in the vertex arrival streaming model where the vertices stream in an arbitrary fashion and assume access to a degree oracle, i.e., we can query for the degree $d_{G} \left(u \right)$ of the vertex $u \in V(G)$ in the stream.

\begin{theorem}\label{theo:sep-vadegubth}
Given any input graph $G = (V, E)$, a coloring function $f : V(G) \rightarrow [C]$ and an input parameter $\vareps > 0$, there exists an algorithm that solves the \colorverify problem in the \vadeg streaming model with high probability in space $\Tilde{\mathcal{O}} \left(\frac{1}{\vareps} \right)$.
\end{theorem}

\begin{proof}
We make use of a reservoir to store $\widetilde{\mathcal{O}} \left(\frac{1}{\vareps} \right)$ edges. Each entry of the reservoir $R$ stores a vertex $u$, it's color $f(u)$, a variable $count$, an integer $b \in [d^{+}_{G}\left(u \right)]$, the vertex $v$ (the $b^{th}$ neighbor of $u$) and it's color $f(v)$. Initially, the reservoir is empty.
The variable $count$ keeps a count of $u's$ successive neighbors seen so far in the stream. $b$ is an integer chosen uniformly at random from $[d^{+}_{G} \left(u \right)]$.

To check if an edge is conflicting, we need to be able to access the colors of both the end points of that edge. Say, $e = (u,v)$ is the edge we want to check for conflict and $u$  appears before $v$ in the stream. While we have access to $v$'s color $f(v)$ when we encounter it in the stream, we have lost the color of $u$, that has already gone past. To deal with this, we use the following approach:
We use reservoir sampling with reservoir size $t$ (where $t = \widetilde{\mathcal{O}} \left(\frac{1}{\vareps} \right))$ to sample $t$ edges independently and uniformly at random. We charge every edge $e=(u,v)$ to the vertex $u$, thus ensuring that no edge is sampled more than once. Every time we see the vertex $u$, we choose its $j^{th}$ neighbor, where $j \in [d^{+}_{G}\left(u \right)]$ chosen uniformly at random. When the $j^{th}$ neighbor of u arrives in the stream, check the colors of both the vertices for conflict. 
\[
\begin{aligned}
 \mathcal{P}(\texttt{an edge e is conflicting}) \geq \frac{\vareps m}{m} = \vareps \\
 \mathcal{P}(\texttt{none of the t edges sampled are conflicting}) \leq \left(1-\vareps \right)^t \leq e^{-\vareps t}
 \end{aligned}
\]
Effectively, we sample $ \Tilde{\mathcal{O}} \left(\frac{1}{\vareps} \right)$ edges. If we get a monochromatic edge in one of our checks, which we get with high probability (i.e. atleast $ \left(1 - n^{-2} \right)$ using Chernoff Bounds) if there are atleast $\vareps m$ conflicting edges, then we can confirm that the coloring is $\vareps$-far from valid. The space complexity of the algorithm is $\Tilde{\mathcal{O}} \left(\frac{1}{\vareps} \right)$.
\end{proof}

%%%%%%%%%% Insert Algorithm %%%%%%%%%%


\begin{algorithm}[]
\SetAlgoLined
\caption{{\sc VA-DegreeOracle-Sep}}
\label{algo:deg-oracle}
\KwIn{$G = (V, E)$ and a coloring function $f$ on $V$ in the \vadeg model}
\KwOut{The algorithm verifies if $f$ is $\vareps$-far from valid or not}

\texttt{Initialize a reservoir } $R$ \texttt{ of size } $t$ \\
    \For{$i \gets 1$ \texttt{ to } $|V|$} { %\comment{loop through the vertices in the stream}
       \texttt{let } $u$ \texttt{ be the } $i^{th}$ \texttt{ vertex of the stream and } $d_{G}(u)$ \texttt{ be its degree}
        \For{$j \gets 1$ \texttt{ to } $t$} { %\comment{loop through the stored vertices in the reservoir}
            \If{$u$ \texttt{ is adjacent to the } $j^{th}$ \texttt{ vertex } $v$ \texttt{ stored in } $R$} {
                \texttt{increment the value of } $v's$ \texttt{ count by } $1$ \\
                \If{$count$ \texttt{ is } $b$ \texttt{(i.e., } $u$ \texttt{ is } $v's$ $b^{th}$ \texttt{ successive neighbor in the stream)} }  {
                    \texttt{store } $u$ \texttt{, along with its color } $f(u)$ \texttt{, as the} $b^{th}$ \texttt{ neighbor of } $v$ \texttt{ (equivalent to storing the edge } $(u,v)$ \texttt{ with their respective colors } $f(u)$ \texttt{ and } $f(v)$ \texttt{ to check if it is monochromatic or not)}
                 }
            }
        %loop through the vertices stored in reservoir R
       }
    %\COMMENT{loop through vertices of the stream}
        \If{$i \leq t$} {
        \texttt{store } $u$ \texttt{ and its color } $f(u)$ \texttt{ and initialize its count to } $0$ \\
        $d^{+}_{G}(u) \gets d_{G}(u) - d^{-}_{G}(u) $ \\
        \texttt{choose } $b$ \texttt{ uniformly at random in the range } $[d^{+}_{G}(u)]$
        }
    	\Else {
        \texttt{with probability } $\frac{t}{i}$ \texttt{, replace an element of the reservoir } $R$ \texttt{, chosen uniformly at random, with } $u$ \texttt{ and its color } $f(u)$ \\
        \texttt{initialize } $u's$ \texttt{ count to } $0$ \\
        \texttt{choose } $b$ \texttt{ uniformly at random from } $[d^{+}_{G}(u)]$ \texttt{(and replace the previous vertex's neighbor, if it has been stored)}
    	}
  }
  \For{$i \gets 1$ \texttt{ to } $t$} {
        \texttt{let } $u$ \texttt{ be the } $i^{th}$ \texttt{ vertex stored in the reservoir } $R$ \texttt{ and } $v$ \texttt{ its stored neighbor (with their respective colors)} \\
        \texttt{check if the assigned the colors to } $u$ \texttt{ and } $v$ \texttt{ make the edge } $(u,v)$ \texttt{ monochromatic}
    }
  \caption{Algorithm: \colorverify in \vadeglong model}
\end{algorithm}

\subsection{\colorverify in \va model} \label{sec:sep-vaaoubsc}

In this variant, we solve the \colorverify problem for graphs in the vertex arrival streaming model.
\begin{theorem}\label{theo:sep-vaaoubth}
Given any input graph $G = (V, E)$, a coloring function $f : V(G) \rightarrow [C]$ and an input parameter $\vareps > 0$, there exists an algorithm that solves the \colorverify problem in the \va streaming model with high probability in space $\widetilde{\mathcal{O}}\left(\min\{\size{V},\frac{|V|^2}{\vareps |E|}\}\right)$.
\end{theorem}

\begin{proof}
We sample independently and uniformly at random the vertices in stream and store these vertices along with their colors. Let $S\subseteq V$ be the set of sampled vertices. When a vertex appears in a stream, we check if it forms a monochromatic edge with one of the stored vertices in $S$. At the end of the stream, the algorithm declares the instance of the graph to be properly colored (valid) if it cannot find a monochromatic edge, else it declares the instance to be $\eps$-far from being monochromatic (valid).
\[
 \mathcal{P}\left(\texttt{an edge e is conflicting}\right) \geq \frac{\vareps m}{ {n \choose 2}} \geq \frac{\vareps m}{n^{2}}
 \]
If we sample $t$ edges overall, independently and uniformly at random, then,
\[
 \mathcal{P}(\texttt{none of the edges sampled are conflicting}) \leq \left(1-\frac{\vareps m}{n^{2}} \right)^t \leq e^{-\frac{\vareps mt}{n^{2}}}
\]
Effectively, we sample $\widetilde{\mathcal{O}}\left(\frac{n^{2}}{\vareps m} \right)$ edges independently and uniformly at random with probability $p=\frac{10\log n}{\sqrt{\vareps m}}$. If one of the sampled edges we check is monochromatic, which we get with high probability (i.e. atleast $ \left(1 - n^{-2} \right)$ using Chernoff Bounds) when there are atleast $\vareps m$ conflicting edges, then we can confirm that the coloring is $\vareps$-far from valid. Otherwise the coloring function is valid.
\end{proof}

%%%%%Algorithm for \conflictest in \varand model

\begin{algorithm}
%\scriptsize

\LinesNumbered

\caption{{\sc Random-Order-Est}($\vareps,T)$: \conflictest in \varandlong model}
\label{algo:random-order}
\KwIn{$G = (V, E)$ and a coloring function $f$ on $V$ in the \varand model, parameters $T$ and $\vareps$.}
\KwOut{$\hat{m}$, that is, a $(1\pm \vareps)$ approximation to $\size{E_M}$.}
%Initialize $\hat{m_h}=0$\.\
Set $t = \lceil \log _{1+\frac{\vareps}{10}}n \rceil$. If $T <63t^2$, then store all the vertices in $G$ along with their colors. At the end, 
report the exact value of $\size{E_M}$. Otherwise, we proceed as follows.\\ 
Let 
\begin{itemize}
\item $\Gamma=\widetilde{\Theta} \left( \frac{n}{\sqrt{T}}\right)$;
\item $v_1,\ldots,v_n$ be the random ordering in which vertices are revealed and $R=\{v_1,\ldots,v_\Gamma\}$;
\item  $\kappa_i, i \in [n],$ denotes the number of monochromatic neighbors of $v_i$ in $R$, that is, 
$\kappa_i = \size{\{(u,v_i): u \in R~\mbox{and}~f(u)=f(v_i)\}}$.
\item $\hat{d_i}, i \in [n],$ denotes the (estimated) monochromatic neighbors of vertices in $G$.\\
\item $H$ denotes the set of \emph{high} degree vertex in $R$, that is, $H=\{v_i:\kappa_i \geq \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8t}\}$
and $L=V \setminus H$;  $L_R=L \cap R$ and $H_R=H \cap R$;
\item The vertices in $L$ are partitioned into $t$ buckets as follows:\\
$B_j=\{v_i \in L: \left(1+\frac{\vareps}{10} \right)^{j-1} \leq d_M(v_i) < \left(1+\frac{\vareps}{10}\right)^{j} \}$, where $j \in [t]$.\\

\end{itemize}

\For{(for each vertex $v_i \in R$ exposed in the stream)}
{
Store $v_i$ as well as its color $f(v_i)$.\\
For each edge $(v_{i'},v_i)$ that arrives in the stream, increase the values of $\kappa_{i'}$ and $\kappa_i$.\\
}
\For{(each $v_i \in R$ with $\kappa_i \geq  \frac{ \size{R}}{n}\frac{\sqrt{\vareps T}}{8t}$)}
{
Add $v_i$ to $H_R$. \\ 
Set $\widehat{d_i}=\frac{n}{\size{R}}\kappa_i$.\\
}
$\widehat{m_h}=\sum\limits_{v_i \in H} \widehat{d_i}$.\\
Let $L_R = R \setminus H_R$. \\
\For{(each $v_i \in L_R$)}
{
Set $\widehat{d_i}=\kappa_i$.\\
}
\For{(for each vertex $v_i \notin R$ exposed in the stream)}
{
Determine the value of $\kappa_i$. If $\kappa_i \geq  \frac{ \size{R}}{n}\frac{\sqrt{\vareps T}}{8t}$, find $\widehat{d_i}=\frac{n}{\size{R}}\kappa_i$ and add $\widehat{d_i}$ to the current $\widehat{m_h}.$ \\
Also, for each $v_{i'} \in L_R$, increase the value of $\widehat{d_{i'}}$ if $(v_{i'},v_i)$ is an edge.\\
}
From the values of $\widehat{d_i}$ for all $v_i \in L_R$, determine the buckets for each vertex in $L_R$. Also, for each $j \in [t]$, find the set $ A_j=\size{L_R \cap B_j}$. Then determine $$\widehat{m_\ell}=\frac{n}{\size{R}}\sum\limits_{ j \in [t]} \size{A_j} \left(1+\frac{\vareps}{10}\right)^i .$$\\
Report $\widehat{m}=\frac{m_h+m_\ell}{2}$ as the final {\sc Output}.
\end{algorithm}


==> query.tex <==
\section{Algorithm for Global Mincut using local queries}
% \remove{\begin{lem}
% \label{lem:highguess}
% Let $G(V,E)$ be a graph, $\hat{t} \geq \frac{10\log ^2 n}{\eps^2}\size{\mbox{\sc Cut}(G)} $ and $\eps \in (0,1)$. If $H(V, E_p)$ be a subgraph of $G$ where each edge in $E(G)$ is included in $E_p$ with probability $p=\min \{\frac{\log n}{\eps^2 \hat{t}},1\}$ independently, then $H$ is diconnected with high probability.
% \end{lem}}

We give a simple and efficient query algorithm in the {\em general graph model} of property testing for estimating the size of the minimum $r$-cut in an unweight and undirected graphs. For an introduction to this model of property testing refer to~\cite[Chapter~10]{G2017}.
In the general graph model of property testing, we can access the graph $G = \left( V(G), E(G) \right)$ using the following "local queries" to the graph $G$:
\begin{itemize}
    \item
        {\bf Degree query:} given $u \in V(G)$, the oracle reports the degree of $u$ in $G$; 

    \item {\bf Neighbor query:} given $u \in V(G)$ and $i \leq |V(G)|-1$, the oracle reports the $i$-th neighbor of $u$, if it exists; otherwise, the oracle reports $\perp$; 

    \item {\bf Adjacency query:}  given a pair of vertices $u, \, v \in V(G)$, the oracle reports whether $\{u,v\} \in E(G)$.
\end{itemize}
The goal is to estimate different parameters in the graph $G$ using as few number of local queries as possible. Using the sampling technique of Karger and Stein~\cite{}, we show the following for global minimum cut in graphs. 

\begin{theo}[Main Result]
There exists an algorithm that has query access to an unknown graph $G$, takes $\eps \in (0,1)$ as input, and computes an $(1 \pm \eps)$ approximation to $t$, that is, the size of the minimum $r$-cut of $G$ with high probability. More over, the number of queries made by the algorithm is $\widetilde{O}\left(\frac{m}{t}\right)$~\footnote{$m$ denotes the number of edges in $G$.}, where each query is a either degree or neighbor query to the graph $G$.
\end{theo}







$\mbox{\sc Cut}_r(G)$--The set of edges in a minimum $r$-cut and $t = |\mbox{{\sc Cut}}_r(G)|$ \\
A graph is denoted by $G(V,E)$ where $|V| = n$ and $|E| = m$. The vertex set of $G$ is often denoted by $V(G)$ and edge set of $G$ is often denoted by $E(G)$. Describe $E_p$ if often used. \\
$\cC_G(A_1,\ldots, A_r)$ -- the cut in $G$ having vertex partition 
$A_1,\ldots, A_r$ with $A_i \neq \emptyset$ for each $i \in [r]$, that 
is, $\cC_G(A_1,\ldots,A_r)=\{(x,y): x \in A_i, y \in A_j~\mbox{and}i \neq 
j\}$.\\
$m_G(A_1,\ldots,A_r)=\size{\cC_G{(A_1,\ldots,A_r)}}$ --  The number edges in the cut $\cC_G{(A_1,\ldots,A_r)}$ in $G$. 




\subsection{To add}


\begin{lem}
\label{lem:highguess}
Let $G(V,E)$ be a graph, $\hat{t} \geq \frac{10 \log n}{\eps^2}\size{\mbox{\sc Cut}_r(G)}$ and $\eps \in (0,1)$. If $H(V, E_p)$ be a subgraph of $G$ where each edge in $E(G)$ is included in $E_p$ with probability $p=\min \{\frac{100r\log n}{\eps^2 \hat{t}},1\}$ independently, then $H$ is connected with probability at most $\frac{1}{10}$.
\end{lem}
\begin{proof}
Let $\cC_G(A_1,\ldots,A_r )$ denote a minimum $r$-cut of $G$.
% , that is, $\mbox{\sc Cut}(G)=\{(x,y): x \in A, y \in V \setminus A\}$. 
As
 we are sampling each edge with probability $p$, the expected size of the $\cC_G(A_1,\ldots,A_r )$ is $p \size{\mbox{Cut}_r(G)} \leq \frac{1}{10 }$. Now applying the Markov's Inequality, we have
 $$ \pr \left(\size{\cC_G(A_1,\ldots,A_r )} \geq 1\right) \leq \E[\size{\cC_G(A_1,\ldots,A_r )}] \leq \frac{1}{10} .$$
 Hence, with probability at most $\frac{1}{10}$, the size of the minimum $r$-cut in $H$ is at least $1$, that is, $H$ is connected.
\end{proof}

\begin{lem}
\label{lem:karger}
Let $G(V,E)$ be a graph, $ \hat{t} \leq \size{\mbox{\sc Cut}_r(G)} $ and $\eps \in (0,1)$. If $H(V, E_p)$ be a subgraph of $G$ where each edge in $E(G)$ is included in $E_p$ with probability $p = \min \{\frac{100r \log n}{\eps^2 \hat{t}},1\}$ independently, then every $r$-cut of size $k$ in $G$ has size $pk(1 \pm \eps)$ in $H$ with probability at least $1-\frac{1}{n^{10}}$.
\end{lem}
\begin{proof}


 
If $p=1$, we are done as the graph $H$ is exactly same as that of $G$. So, with out loss of generality assume that the graph $G$ has at most $r-1$ connected components. Otherwise, the lemma holds trivially as $\size{\mbox{\sc Cut}_r(G)} =0$, that is, $\hat{t}=0$ and $p=1$. Hence, we assume that $p=\frac{c'\log n}{\eps^2 \hat{t}}$ for the rest of the proof.

If a $r$-cut of size $k$ in $G$ has size $pk(1 \pm \eps)$ in $H$, then we say
the $r$-cut is approximately preserved in $H$. Consider a $r$-cut $\cC_G(A_1,\ldots,A_r)$ of size $k$ in $G$. As we are sampling each edge with probability $p$, the expected size of the  $\cC_H(A_1,\ldots,A_r)$ is $pk$. Using Chernoff bound(See Lemma ~\ref{lem:cher_bound1} in Section~\ref{sec:append}), the probability that  $\cC_H(A_1,\ldots,A_r)$ is not approximately preserved is given by
 \begin{equation}\label{eq:cher}
     \pr \left(\size{\mbox{$\cC_H(A_1,\ldots,A_r)-pk$}} \geq \eps pk  \right) \leq e^{-\eps^2pk/3\hat{t}} 
             = n^{-\frac{100k}{3\hat{t}}}
 \end{equation}
 Now, we will use the following bound on the number of cuts of a particular size.
\begin{lem}[~\cite{Karger93}]
\label{lem:karger_cut_bound}
Let $OPT>0$ be the size of any minimum $r$-cut in a graph $G$. Then the number of $r$-cut in a $G$ having at most a factor $j\cdot OPT$ is at most $n^{2j (r-1)}$.
\end{lem}
% \begin{proof}
Now, let $Z_1,Z_2,\ldots,Z_{\ell}$ be the partition of the set of all  $r$-cuts in $G$ such that each $r$-cut in $Z_j$ has number of edges between $[j\cdot OPT,(j+1)OPT]$, where $\ell \leq \frac{n}{OPT}$ and $j \leq \ell-1$. From Lemma~\ref{lem:karger_cut_bound}, $\size{Z_j} \leq n^{2j(r-1)}$. Consider a  particular $Z_j, j \in [\ell]$. Using the union bound along with Equation~\ref{eq:cher}, the probability that there exists a $r$-cut in $Z_j$ that is not approximately preserved in $H$ is at most $\frac{1}{n^{11}}$. Taking union bound over all $Z_j$'s, the probability that there exists a $r$-cut in $G$ that is not approximately preserved is at most $\frac{1}{n^{10}}.$
\end{proof}



% \begin{theo}[tail bounds to be put in appendix]
% \label{theo:chernoff_bounds1}
% Let $X := \sum_{i \in [n]}X_i$ such that $X_i$, $i \in [n]$, are independently distributed on $[0,1]$. Then for all $\epsilon > 0$
% \[
%     \pr\left(|X - \mathbb{E}X| \geq \epsilon\mathbb{E}X\right) \leq e^{-\eps^2 \mathbb{E}X/3}
% \]
% \end{theo}

\subsection{Algorithm for global mincut}

\begin{algorithm}[H]
\SetAlgoLined
\caption{{\sc Sample}(${ D},p)$}
\label{algo-sample}
\KwIn{${ D}=\{d_i: i \in [n] \}$, where $d_i$ denotes the degree of the $i$-th vertex in the graph $G$ and $m=\frac{1}{2}\sum\limits_{i=1}^{n}d_i \geq n-1$. Also, $p \in (0,1]$.}
\KwOut{Return a subgraph $H(V,E_p)$ of $G(V,E)$ where each edge in $E(G)$ is included in $E_p$ with probability $p$.}
\remove{Find $m=\frac{1}{2}\sum \limits_{i=1}^{d_i}$.\\
\If{($p \geq \frac{100 \log n}{m}$)}
{
{\sc Find All the edges:} Extract the entire graph $G$ by using $D$ along with neighbor queries. Determine $\mbox{{\sc Cut }}_r(G)$ and return $G(V,E)$ as $H(V,E_p)$.
}}
Set $q=1-\sqrt{1-p}$ and $m=\frac{\sum_{i=1}^nd_i}{2}$ \\
\For{(each $i \in [n]$)}
{
\For{(each $j \in [d_i]$)}
{
Ask for the $j$-th neighbor of $i$-the vertex with probability $q$. \\
Let $r_j \in [n]$ be the $j$-the neighbor of $i$ if it is asked. In that case, add the edge $(i,r_j)$ to $E_p$. %\footnote{\textcolor{red}{Is this clear?}} \\
\If{($\size{E_p} \geq  2pm  $)} 
{return {\sc Fail}.}
}
Return the graph $H(V,E_p)$.
}
\end{algorithm}

\begin{lem}
\label{lem:sample_dp_lemma}
With probability at least $1-\frac{1}{n^{10}}$, {\sc Sample}$(D,p)$ returns a random subgraph $H(V,E_p)$ of $G(V,E)$ such that each edge $e \in E$ is included in $E_p$ with probability $p$. More over,  {\sc Sample}$(D,p)$ makes ${O}(pm)$ many neighbor queries to the graph $G$.
\end{lem}
\begin{proof}
From the description of {\sc Sample}($D,\eps$), it is clear that 
the probability that a particular edge $e \in E(G)$ is added to $E_p$ with probability $1-(1-q)^2=p$. So, the expected size of $E_p$ is $pm$. Now, by Chernoff bound (See Lemma~\ref{lem:cher_bound1} in Section~\ref{sec:append}), we have 
$$\pr\left( \size{E_p} \geq 2 pm\right) \leq e^{-\frac{pm}{3}} \leq \frac{1}{n^{10}}. $$
The last inequality holds because $pm = \min\{\frac{c' \log n}{\eps^2 \hat{t}},1\} \times m \geq 10 \log n$ as $m \geq n-1$ and $\hat{t} \leq \frac{n}{2}$.

The number of neighbor queries made by {\sc Sample}($D,\eps$) is $\size{E_p} ={O}{(pm)}$ as we make one query per each edge in $E_p$.
\remove{
{\sc Sample}($D,\eps$) makes expected $O(qd_i)$ queries for each vertex $i \in [n]$ and thus total number of expected queries is $O(pm)$ whp. Fix an edge $(i,j) \in E(G)$. We show that probability $(i,j)$ is sampled is $p$.
\begin{align*}
    \pr\left( (i,j) \text{ is sampled}\right) &= 1 - \pr\left( (i,j) \text{ is not sampled}\right) \\
    &= 1 - (1-q)^2 \\
    &= p
\end{align*}}
\end{proof}



\begin{algorithm}[H]
\SetAlgoLined
\caption{{\sc Verify-Guess}(${ D},\hat{t},\eps$)}
\label{algo}
\KwIn{${ D}=\{d_i: i \in [n] \}$, where $d_i$ denotes the degree of the $i$-th vertex in the graph $G$ and $m=\frac{1}{2}\sum\limits_{i=1}^{n}d_i > n-1$. Also, a guess $\hat{t}$, with $1 \leq \hat{t} \leq \frac{n}{2}$, for the size of the global mincut in $G$, and $\eps \in (0,1)$.}
\KwOut{Accept or reject $\hat{t}$. If it accepts, return an estimate for $\tilde{t}$ for $\size{\mbox{\sc Cut}_r(G)}$.}
Set $p=\min \{\frac{100r\log ^2 n}{\eps^2 \hat{t}},1\}$. \\
Set $\Gamma=100 \log n $ and Call {\sc Sample}($D,p$) $\Gamma$ times.\\
If at least one {\sc Sample}($D,p$) returns {\sc Fail}, then
Return {\sc Fail} as the output of {\sc Verify-Guess} and {\sc Quit}. \\
Otherwise, Let $H_i(V,E^i_p)$ be the output of $i$-th call to {\sc Sample}($D,p$), where $i \in [\Gamma]$\\
\If{$\left(\mbox{At least}~\frac{\Gamma}{2} ~\mbox{many}~ H_i's\mbox{ are disconnected}\right)$}
{ Reject $\hat{t}$}
\ElseIf{(All $H_i$'s are connected)}
{Accept $\hat{t}$, find $\mbox{{\sc Cut}}_r(H_i)$ for any $i \in [\Gamma]$, and return $\tilde{t}= \frac{ \size{\mbox{{\sc Cut}}_r(H_i)}}{p}$.}
\Else {
Return {\sc Fail}.
}
%\LinesNumbered
\end{algorithm}

\begin{lem}
\label{lem:guess}
{\sc Verify-Guess}$(D,\hat{t},\eps)$ makes $\widetilde{O}\left(\frac{mr }{\hat{t}} \right)$ many neighbor queries to the graph $G$ and behaves as follows.
\begin{itemize}
    \item[(i)] If $\hat{t} \geq \frac{10 \log n}{\eps^2}\size{\mbox{{\sc Cut}}_r(G)} $, then  {\sc Verify-Guess}$(D,\hat{t},\eps)$ rejects $\hat{t}$ with probability at least $1-\frac{1}{n^{9}}$,
      \item[(ii)] If $\hat{t} \leq \size{\mbox{{\sc Cut}}_r(G)} $, then {\sc Verify-Guess}$(D,\hat{t},\eps)$ accepts $\hat{t}$ with probability at least $1-\frac{1}{n^{9}}$. Moreover, in this case, {\sc Verify-Guess}$(D,\hat{t},\eps)$ reports an $(1 \pm \eps)$-approximation to $\mbox{{\sc Cut}}_r{(G)}$. 
\end{itemize}
\end{lem}
\begin{proof}
 {\sc Verify-Guess}$(D,\hat{t},\eps)$ calls {\sc Sample}($D,\eps$) for $\Gamma=100 \log n$ times with $p$ being set to $\min \{\frac{100 r\log ^2 n}{\eps^2 \hat{t}},1\}$. Recall Lemma~\ref{lem:sample_dp_lemma}. Each call to {\sc Sample}($D,\eps$) makes $O(pm)$ many neighbor queries and returns a random subgraph $H(V,E_p)$ with probability at least $1-\frac{1}{n^{10}}$, where each edge in $E(G)$ is included in 
 $E_p$ with probability $p$. So, {\sc Verify-Guess}$(D,\hat{t},\eps)$ 
 makes  ${O}(pm \log n)=\widetilde{O}\left( \frac{mr}{\hat{t}}\right)$ many 
 neighbor queries and generate $\Gamma$ many random subgraphs with
 $H_1(V,E_p^1),\ldots,H_{\Gamma}(V,E_p^{\Gamma})$ probability at least $1-\frac{\Gamma}{n^{10}}$.
 \remove{ If the value of $p$ is $1$ then {\sc Verify-Guess}$(D,\hat{t},\eps)$ makes at most 
% $O(n + m)$ 
$O(m)$ neighbour queries and other hand is value of $p$ is $\frac{10\log  n}{\eps^2 \hat{t}}$, then {\sc Verify-Guess}$(D,\hat{t},\eps)$ makes at most ${O}\left(\frac{m\log ^2 n}{\eps ^2\hat{t}} \right)$ neighbour queries.}

\remove{Again by Lemma\ref{lem:sample_dp_lemma}, {\sc Sample}($D,\eps$) returns a random subgraph $H(V,E_p)$, with probability at least $1-\frac{1}{n^{10}}$, such that each edge in $E(G)$ is included in $E_p$ with probability $p$.}

\begin{description}
\item[Proof of (i)] Here $\hat{t} \geq \frac{10\log n}{\eps^2}\size{\mbox{{\sc Cut}}_r(G)}$. Applying Lemma~\ref{lem:highguess}, $H_i$ is connected with probability at most $\frac{1}{10}$ for any particular $H_i$. So, The expected number of $H_i$ that are disconnected is at least $\frac{9\Gamma}{10}$. By Chernoff bound(See Lemma~\ref{lem:cher_bound1} in Section~\ref{sec:append}), the probability that at most $\frac{\Gamma}{2}$ many $H_i$'s are disconnected is at most $\frac{1}{n^{10}}$. Hence, {\sc Verify-Guess}$(D,\hat{t},\eps)$ rejects any $\hat{t}$ satisfying $\hat{t} \geq \frac{10 \log n}{\eps^2}\size{\mbox{{\sc Cut}}_r(G)}$, with probability at least $1-\frac{1}{n^{9}}$.   
\item[Proof of (ii)]  Here $\hat{t} \leq \size{\mbox{{\sc Cut}}_r(G)}$. Applying Lemma~\ref{lem:karger}, we have every cut of size $k$ in $G$ has size $pk(1 \pm \eps)$ in $H_i$ with probability at least $1-\frac{1}{n^{10}}$ for any particular $H_i$. Hence, the probability that in any $H_i, i \in [\Gamma],$ every cut of size $k$ in $G$ has size $pk(1 \pm \eps)$ is at least $1-\frac{\Gamma}{n^{10}}$. So,  {\sc Verify-Guess}$(D,\hat{t},\eps)$ accepts any $\hat{t}$ satisfying $\hat{t} \leq \size{\mbox{{\sc Cut}}_r(G)}$, with probability $1-\frac{1}{n^{9}}$. More over, for any $H_i$, observe that $\frac{\size{\mbox{{\sc Cut}}_r(H_i)}}{p}$ is an $(1 \pm \eps)$-approximation to $\size{\mbox{{\sc Cut}}_r(H)}$. Hence, when $\hat{t} \leq \size{\mbox{{\sc Cut}}_r(G)}$, {\sc Verify-Guess}$(D,\hat{t},\eps)$ also returns an $(1\pm \eps)$ approximation to $\size{\mbox{\sc Cut }(G)}$ with probability $1-\frac{1}{n^9}$.
\end{description}
\remove{Now,

\emph{Proof of (i)} from

\emph{Proof of (ii)}}
\end{proof}

\begin{algorithm}[H]
\SetAlgoLined
\caption{{\sc Estimator}($\eps$)}
\label{algo-estimator}
\KwIn{An $\eps \in (0,1)$ along with the degree and neighbor query access to $G$.}
\KwOut{An $(1 \pm \eps)$-approximation to $t=\size{\mbox{{\sc Cut}}_r(G)}$.}
Find the degrees of all the vertices in $G$ by making $n$ many degree queries. Let $D=\{d_1,\ldots,d_n\}$, where $d_i$ denotes the degree of the $i$-the vertex in $G$.\\
Find $m=\frac{1}{2} \sum \limits _{i=1}^n d_i$. If $m<n-1$, return $t=0$ and {\sc Quit}. Otherwise, proceed as follows.\\
Set $\kappa=\frac{10 \log  n}{\eps^2}$\\
Initialize $\hat{t}=\frac{n}{2}$.\\
\While{($\hat{t} \geq 1$)}
{
Call {\sc Verify-Guess}($D,\hat{t},\eps$). \\
\If{({\sc Verify-Guess} returns {\sc Fail})}
{Return {{\sc Fail}} as the output of {{\sc Estimator}}($\eps$)}
\ElseIf{({\sc Verify-Guess} rejects $\hat{t}$)}
{set $\hat{t}=\frac{\hat{t}}{2}$ and continue.}
\Else { 
Set $\hat{t_u} =\max \{\frac{\hat{t}}{\kappa},1\}$.\\ 
Call {\sc Verify-Guess}($D,\hat{t_u},\eps$) \\
If  {\sc Verify-Guess} returns {\sc Fail} or reject $\hat{t_u}$, then 
return {\sc Fail} as the output of {\sc Estimator}($\eps$).
Otherwise, let $\tilde{t}$ be the output of {\sc Verify-Guess}. \\
Return $\tilde{t}$ as the output of {\sc Estimator}($\eps$).

}
}
%{\sc Find All the edges:} Extract the entire graph $G$ by using $D$, that is, the degree information of all the vertices along with neighbor queries. Determine $\mbox{{\sc Cut }}(G)$ and return $\size{\mbox{{\sc Cut }}(G)}$.
{\bf Output:} Return that the graph $G$ is disconnected.

\end{algorithm}



\begin{lem}\label{thm:main}
{\sc Estimator}($\eps$) returns $(1 \pm \eps)$ approximation to $\size{\mbox{{\sc Cut}}_r(G)}$ with probability at least $1-\frac{1}{n^8}$ by making $\widetilde{O} \left(\frac{mr}{t}\right)$ queries, where $t=\size{\mbox{{\sc Cut}}_r(G)}$ and each query is either a degree or a neighbor query to the graph $G$.
\end{lem}
\begin{proof}
With out loss of generality, assume that $n$ is a power of $2$. If $m < n-1$ then the graph $G$ is disconnected. In this case the algorithm {\sc Estimator}($\eps$) makes $O(n)$ degree queries and returns the correct answer deterministically. Thus we assume that $m\geq n-1$. 

First, we prove the correctness and query complexity when the graph is
connected, that is, $t\geq 1$. Note that {\sc Estimator}($\eps$) calls
{\sc Verify-Guess}($D,\hat{t},\eps$) for different values of $\hat{t}$ starting from $n$. Recall that $\kappa=\frac{10 \log n}{\eps^2}$. For a particular $\hat{t}$ with $\hat{t}\geq \kappa t$, {\sc Verify-Guess}($D,\hat{t},\eps$) accepts $\hat{t}$ with probability at
most $\frac{1}{n^{9}}$ by Lemma~\ref{lem:guess}~(i). So, by the union bound, the probability that {\sc Verify-Guess}($D,\hat{t},\eps$) accepts some $\hat{t}$ with $\hat{t}\geq \kappa t$, is at most $\frac{\log n}{n^{9}}$. Hence, with probability at least
$1-\frac{\log n}{n^{9}}$, we can say that the {\sc Verify-Guess}($D,\hat{t},\eps$) rejects all $\hat{t}$ with $\hat{t}\geq \kappa t$. As $t \geq 1$, there exists a $\hat{t}$ with $ \frac{t}{2} <\hat{t} \leq t$ such that if we call {\sc Verify-Guess}($D,\hat{t},\eps$), it will accept $\hat{t}$ with
probability at least $1-\frac{1}{n^{9}}$ by lemma~\ref{lem:guess} (ii). Putting together, {\sc Estimator}($\eps$) accepts a $\hat{t}$ with $ \frac{t}{2}< \hat{t} < \kappa t$ with probability $1-\frac{\log n +1}{n^{9}}$. From the description of {\sc
Estimator}($\eps$), note that, we find $\hat{t_u}$ by dividing $\hat{t}$ by $\kappa$. Now,  we have $\hat{t_u} < t$ and we run the {\sc Verify-Guess}($D,\hat{t_u},\eps$) with $\hat{t_u}$. By
Lemma~\ref{lem:guess}~(ii), {\sc Verify-Guess}($D,\hat{t},\eps$) accepts and reports an $(1\pm \eps)$ approximation to $t$ with probability at least $1-\frac{1}{n^{9}}$. Now we analyze the number
of queries made by the algorithm. We make an initial $n$ many queries to construct $D$. Then at the worst case, we call {\sc Verify-Guess}($D,\hat{t},\eps$) for $\hat{t}=n,\frac{n}{2},\ldots
,t'$ and $\hat{t_u}=\frac{t'}{\kappa} \geq \frac{t}{2\kappa}$, where $ \frac{t}{2}< t' <\kappa t$. It is because 
{\sc Verify-Guess}($D,\hat{t},\eps$) accepts $\hat{t}$ with probability $1-\frac{1}{n^{9}}$ when $\hat{t}\leq t$. Hence, by Lemma~\ref{lem:guess}, the total number of queries made by the algorithm is $O\left(n+ \log n \cdot \widetilde{O}\left(\frac{mr }{  \hat{t_u}} \right)\right)$, where each query is either a degree or a neighbor query. Note that $n \leq \frac{mr}{t}$ as $t \geq 1$. Also $\hat{t_u}\geq \frac{t}{2 \kappa}$. Hence, the total number of queries made by {\sc Estimator}{($\eps$)}, when $t \geq 1$, is $\widetilde{O}\left( \frac{mr}{t}\right)$. 


Now we analyze the case when $t=0$, {\sc Verify-Guess}($D,\hat{t},\eps$) rejects all $\hat{t} \geq 1$ with probability $1-\frac{\log n}{n^{9}}$. Then, in {\sc Estimator}($\eps$) reports $t=0$. As we have called {\sc Verify-Guess}($D,\hat{t},\eps$) for all $\hat{t}=\frac{n}{2},\ldots,1$, the number of queries made by {\sc Estimator}($\eps$), in the case when $t=0$, is $\widetilde{O}(m)$.
\end{proof}

\subsection{Finding exact minimum cut}

\begin{theo}[Local and random queries and finding minimum cuts]
        Let us assume that the query algorithms have access to {\sc degree}, {\sc neighbour}, {\sc adjacency} and {\sc random edge} queries to an an unknown graph $G = (V(G), E(G))$ with $\size{V(G)} = n$ and $\size{E(G)} = m$. 
        Also, let $t \in \mathbb{N}$ with $m \geq 2tn$. Any query algorithm that can decide if the minimum cut in $G$ is $t$ or $t-1$, with probability at least $2/3$, will require $\Omega\left(m \right)$ many queries. 
\end{theo}
\begin{proof}
    \textcolor{red}{Arijit: To be added.}
\end{proof}

Now we will show that using induced degree query, we can find exact minimum cut efficiently. 

We will assume that $0< \eps \leq 1/5$, and we have an estimate $\hat{t}$ of the minimum cut value $\size{\mbox{{\sc Cut}}_{2}(G)}$\footnote{\textcolor{red}{Arijit: I will write the calculation for $r=2$ today. If the calculations goes through}} satisfy the following:
$$
    \frac{1}{1+\eps}\leq \frac{\hat{t}}{\size{\mbox{{\sc Cut}}_{2}(G)}} \leq 1+\eps
$$
Note that we can find such an estimate for $\size{\mbox{{\sc Cut}}_{2}(G)}$ using the algorithms in the previous section using $\widetilde{\mathcal{O}}\left( \frac{m}{t}\right)$ many local queries where $t = \size{\mbox{{\sc Cut}}_{2}(G)}$.  

The following theorem shows the hardness of finding the minimum cut using local and random edge queries. 






Without loss of generality, assume that the minimum cut is not a singleton cut in the graph. 


\begin{algorithm}
\SetAlgoLined
\caption{{\sc Finding exact minimum cut}($\eps$)}
\label{algo-exact-min-cut}
\KwIn{Induced degree access to the graph $G$.}
\KwOut{Exact minimum cut $\mbox{{\sc Cut}}_{2}(G)$ of $G$.}
\begin{description}
    \item[Step 1.]
        Sample each edge of $G$ with probability $p = \min\left\{ \frac{200(1+\eps)\log n}{\eps^{2} \hat{t}}, \, 1\right\}$ to obtain the subgraph $\widetilde{G}= (V, E_{p})$ of $G$.
    
    
    \item[Step 2.]
        Compute all non-singleton cuts in $\widetilde{G}$ of size at most $(1+\eps)p\hat{t}$. 
        
    \item[Step 3.]
    We will now construct a partition of the vertex set $V$ using the cuts computed in {\bf Step 2}.
    Contract any two
        vertex belongs to the same partition if they are together in all such cuts computed in {\bf Step 2}. 
    Without loss of generality, let the partition of $V$ be $V = \cup_{i=1}^{t} V_{i}$ for some $t \in [n]$. 
    
    
    \item[Step 4.]
        We will now construct a new multigraph $\widehat{G}$ whose vertex set is $\{V_{1}, \, \dots, \, V_{t}\}$ and the edges corresponds to the edges in $G$ going across all $V_{i}$ and $V_{j}$ where $i, \, j \, (i\neq j) \in [t]$. We learn all the edges in $\widehat{G}$ using induced degree queries, unless the number of edges in $\widehat{G}$ becomes more than $n\log n$, in which case we report a ``Failure'' and terminate the algorithm. 
        
    \item[Step 5.] Output the minimum cut in the graph $\widehat{G}$.
\end{description}
\label{algorithm-finding-mincut}
\end{algorithm}

We will now prove the following theorem. 

\begin{theo}[Separating local and induced degree queries]
    Algorithm~\ref{algo-exact-min-cut} computes the minimum cut using $\widetilde{\mathcal{O}}\left( \frac{m}{t}\right)$, where $m = \size{E}$ and $t = \mbox{{\sc Cut}}_{2} \left( G\right)$, with probability at least $1-\frac{1}{n^{10}}$.
    \label{thm:induced-degree-mincuts}
\end{theo}
\begin{proof}
    We will first prove the correctness of the algorithm.
    Observe that from Lemma~\ref{}, with probability at least $1 - \frac{1}{n^{10}}$, all cuts $\mbox{Cut}^{2}_{G}(A_{1}, A_{2})$ satisfy the following inequality:
    $$
        (1-\eps)p \leq
        \frac{\size{\mbox{{\sc Cut}}^{2}_{\widetilde{G}}(A_{1}, A_{2})}}{\size{\mbox{{\sc Cut}}^{2}_{{G}}(A_{1}, A_{2})}}
        \leq (1+\eps)p.
    $$
    Also, note that this implies that if $\size{\mbox{{\sc Cut}}^{2}_{\widetilde{G}} (A_{1}, A_{2})} \leq (1+\eps)p\hat{t}$, then $\size{\mbox{{\sc Cut}}^{2}_{\widetilde{G}} (A_{1}, A_{2})} \leq (1+4\eps)\mbox{{\sc Cut}}_{2}(G)$. Note that, from Theorem~\ref{prop-KawarabayashiT15}, this implies that ``Failure'' case in {\bf Step 4} of Algorithm~\ref{algorithm-finding-mincut} does not happen with probability at least $1 - \frac{1}{n^{10}}$.
    Therefore Algorithm~\ref{algorithm-finding-mincut} computes the exact minimum cut with probability at least $1-\frac{1}{n^{10}}$.
    
    Observe that using $O\left( \log n\right)$ many induced degree queries we can simulate the $j$-neighbor query of a vertex. Using Lemma~\ref{algorithm-finding-mincut} together with this observation, we can implement {\bf Step 1} of Algorithm~\ref{algorithm-finding-mincut} using $\widetilde{\mathcal{O}}\left( \frac{m}{t}\right)$ many induced degree queries. For {\bf Step 2} and {\bf Step 3} of the Algorithm~\ref{algorithm-finding-mincut} we are not using any induced degree queries. For {\bf Step 4} of the Algorithm~\ref{algorithm-finding-mincut}, observe that, using Lemma~\ref{lem-finding-all-neighbors-induced-degree} and the fact that $n \leq \frac{m}{t}$, we will be using using $\widetilde{\mathcal{O}}\left( n\right) = \widetilde{\mathcal{O}}\left( \frac{m}{t} \right)$ many induced degree queries. Putting together everything, the total number of induced queries used by our algorithm will be bounded by $\widetilde{\mathcal{O}}\left( \frac{m}{t}\right)$.
\end{proof}

To completely the proof of Theorem~\ref{thm:induced-degree-mincuts} we will need the following two results. 

\begin{theo}[Kawarabayashi and Thorup~\cite{KawarabayashiT15}]
    Let $G = (V(G), E(G))$ with minimum degree $d$ and minimum cut value $c$. For $\eps \in [0,1)$, let $\mathcal{C}(\eps)$ be the family of all non-singleton cuts in the graph in $G$ with cut value at most $c + \eps d$. Then number of edges of $G$ that is participating in at least one of the cuts from $\mathcal{C}({\eps})$ is bounded by $O(n)$.
    \label{prop-KawarabayashiT15}
\end{theo}

\begin{lem}\label{lem-finding-all-neighbors-induced-degree}
        Let us assume that the query algorithms have access to {\sc induced degree} query to an unknown graph $G = (V(G), E(G))$. 
        There exists an algorithm that takes as input a subset $S$ of $V(G)$ and $v \in V(G)$, and outputs the set $S\cap N(v)$ using $\mathcal{O}\left(\size{S\cap N(v)}\log n\right)$ many queries, where $n = \size{V(G)}$.
\end{lem}
\begin{proof}
    
\end{proof}

==> random.tex <==
%\section{Upper bound for estimating the number of monochromatic edges when vertices arrive in a random order}
%\subsection{\conflictest in \varandlong} \label{sec:est-varandlong1}
\section{\conflictest in \varand model}\label{sec:est-vardubsc}%\label{sec:vardub}
In this Section, we show that the power of randomness can be used to design a better solution for the \conflictest problem in the \varand model. The \conflictest problem is the main highlight of our work. We feel that the crucial use of randomness in the input that is used to estimate a substructure (here, monochromatic edges) in a graph, will be of independent interest.

%\subsection{\conflictest in \varand model} \label{sec:est-vardubsc}
 In this variant, \remove{we solve the \conflictest problem in the vertex arrival model when vertices stream in a random order.}we are given an $ \vareps \in (0,1)$ and a promised lower bound $T$ on $\size{E_M}$, the number of monochromatic edges in $G$, as input and our objective is to determine a $(1 \pm \vareps)$-approximation to $\size{E_M}$. 
 
 \begin{theorem} \label{theo:est-vardubth}
 Given any graph $G=(V,E)$ and a coloring function $f: V(G) \rightarrow [C]$ as input in the stream, the \conflictest problem in the \varand model can be solved with high probability in $\widetilde{\mathcal{O}} \left(\frac{\size{V}}{\sqrt T} \right)$ space, where $T$ is a lower bound on the number of monochromatic edges in the graph.  \end{theorem}

{Let $v_1,\ldots,v_n$ be the random ordering in which the vertices of $V$ are revealed.} Let $R$ be a random subset of 
$\Gamma=\widetilde{\Theta}\left( \frac{n}{\sqrt{T}}\right)$~\footnote{$\Theta(\cdot)$ hides a polynomial factor of $\log n$ and $\frac{1}{\vareps}$ in the upper bound.} many vertices of $G$ sampled without replacement. 
As we are dealing with a random order stream, consider the first $\Gamma$ vertices in the stream; they can be treated as $R$, the random sample. We start by storing all the vertices in $R$ as well as their colors. 
Observe that the monochromatic degree of any vertex $v_i$, if it is \emph{large} (say roughly more than $\sqrt{T}$), can be well approximated by looking at the number of monochromatic neighbors that $v_i$ has in $R$.
\remove{Observe that \comments{the monochromatic degree} of any vertex $v_i$, having \emph{large} (say roughly more than $\sqrt{T}$) monochromatic degree, can be well approximated by looking at the number of monochromatic neighbors that $v_i$ has in $R$.}As a vertex $v_i$ streams past, there is no way we can figure out its monochromatic degree, unless we store its monochromatic neighbors that appear before it in the stream; if we could, we were done. Our only savior is the stored random subset $R$. Our algorithm proceeds by figuring out the influence the color of $v_i$ has on the monochromatic degrees of vertices in $R$.
To estimate this, let $\kappa_i$ denote the number of monochromatic neighbors that $v_i$ has in $R$. We set a threshold $\tau=\frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8t}$, where $t=\lceil \log _{1+\frac{\vareps}{10}} n\rceil$. The significance of $t$ will be clear from the discussion below. Any vertex $v_i$ will be classified as a \emph{high} or \emph{low} degree vertex depending on its monochromatic degree within $R$, i.e., 
whether $\kappa_i \geq \tau$ or not, respectively. Let $H$ and $L$ be the set of high and low degree vertices in $G$. Let $H_R$ and $L_R$ denote the set of high and low degree vertices in $R$. Notice that, because of the definition of high and low degree vertices, not only the sets $H_R, \, L_R \subseteq R$, but they are determined by the vertices of $R$ only.

Let $m_h$ and $m_\ell$ denote the sum of the monochromatic degrees of all the high degree vertices and low degree vertices in $G$, respectively. 
So, $m_h=\sum\limits_{v \in H}d_M(v)$ and $m_\ell=\sum\limits_{v \in L}d_M(v)$. Note that $ \widehat{m} = \size{E_M} =\frac{1}{2}\sum_{v \in V} d_M(v) = \frac{1}{2}\left( m_h+m_\ell\right).$
We will describe how to approximate $m_h$ and $m_\ell$ separately. The formal algorithm is described in Algorithm~\ref{algo:random-order} as {\sc Random-Order-Est}$(\vareps,T)$ (in the Appendix) that basically executes steps to approximate $m_h$ and $m_\ell$ in parallel.

\noindent
{\bf Approximating $m_h$:} 
 %\paragraph*{Approximating $m_h$:} 
 We can find $\widehat{m_h}$, that is, a $\left( 1\pm \frac{\vareps}{10}\right)$ approximation of $m_h$ as described below. For each vertex $v_i \in R$ and each monochromatic edge $(u,v_i)$ we see in the stream, we increase the value of $\kappa$ for both $u$ and $v_i$. After all the vertices in $R$ are revealed, we can determine $H_R$ by checking whether $\kappa_i \geq \tau$ for each $v_i \in R$. For each vertex $v_i \in H_R$, we set its approximate monochromatic degree $\widehat{d_i}$ to be $\frac{n}{\size{R}}\kappa_i$. We initialize the estimated sum of the monochromatic degree of high degree vertices as $\widehat{m_h}=\sum\limits_{v_i \in H_R}\widehat{d_i}$. For each vertex $v_i \notin R$ in the stream, we can determine $\kappa_i$, as we have stored all the vertices in $R$ along with their colors, and hence we can also determine whether $v_i$ is a high degree vertex in $G$. If $v_i \notin R$ is a high degree vertex, we determine $\hat{d_i}=\frac{n}{\size{R}}\kappa_i$ and update $\widehat{m_h}$ by $\widehat{m_h}+\hat{d_i}$. Observe that, at the end, $\widehat{m_h}$ is $\sum\limits_{v_i \in H}\widehat{d_i}$. Recall that $H$ is the set of all high degree vertices in $G$. For each $v_i \in H$, we will show that $\widehat{d_i}$ is a $\left(1\pm \frac{\vareps}{10}\right)$-approximation to $d_M(v_i)$ with high probability. This implies that 
 \begin{center}
\begin{equation}
\label{eqn:high-over}
 \left(1-\frac{\vareps}{10}\right)m_h \leq \widehat{m_h} \leq \left(1+\frac{\vareps}{10}\right)m_h
\end{equation}
\end{center}
 
 \noindent
 {\bf Approximating $m_\ell$:}
 %\paragraph*{Approximating $m_\ell$:} 
 Recall that $m_\ell=\sum\limits_{v_i \in L}d_M(v_i)$. Unlike the high degree vertices, it is not possible to approximate the degree of $v_i \in L $ from $\kappa_i$. \remove{Note that $\kappa_i$ is the number of monochromatic neighbors that $v_i$ has in $R$.} To cope up with this problem, we partition the vertices of $L$ into $t$ buckets $B_1,\ldots,B_t$ such that all the vertices present in a bucket have \emph{similar} degrees, where $t=\lceil \log _{1+\frac{\vareps}{10}} n\rceil$. The bucket $B_j$ is defined as follows: $B_j=\{v_i\in L: \left(1+\frac{\vareps}{10} \right)^{j-1} \leq d_M(v_i) < \left(1+\frac{\vareps}{10}\right)^{j} \}$.

 %\[B_j=\{v_i\in L: \left(1+\frac{\vareps}{10} \right)^{j-1} \leq d_M(v_i) < \left(1+\frac{\vareps}{10}\right)^{j} \}\]
 
 Note that our algorithm will not find the buckets explicitly. It will be used for the analysis only. Observe that 
 $\sum\limits_{j \in [t]}\size{B_j}\left( 1+\frac{\vareps}{10}\right)^{j-1} \leq  m_\ell  < \sum\limits_{j \in [t]}\size{B_j}\left( 1+\frac{\vareps}{10}\right)^{j}$. 
 %\[ \sum\limits_{j \in [t]}\size{B_j}\left( 1+\frac{\vareps}{10}\right)^{j-1} \leq  m_\ell  < \sum\limits_{j \in [t]}\size{B_j}\left( 1+\frac{\vareps}{10}\right)^{j} \]
  We can surely approximate $m_\ell$ by approximating $\size{B_j}$s suitably. We estimate $\size{B_j}$s as follows.\remove{ However, we will be able to have a $\left(1+\frac{\vareps}{10}\right)$-approximation of $\size{B_j}$, with high probability, if $\size{B_j}\geq \frac{\sqrt{\vareps T}}{10t}$ as follows.} After the stream of the vertices in $R$ has gone past, we have the set of low degree vertices $L_R$ in $R$ and $\widehat{d_i}=\kappa_i$ for each $v_i \in L_R$. For 
  each $v_i \notin R$ in the stream, we determine the monochromatic neighbors of $ v_i$ in $L_R$. It is possible as we have stored all the 
  vertices in $R$ and their colors. For each monochromatic neighbor $v_{i'}\in L_R$ of $v_i$, we increase the value of  $\widehat{d}_{i'}$ 
  of $v_{i'}$.  Observe that, at the end of the stream, $\widehat{d_{i'}}=d_M(v_{i'})$ for each $v_{i'} \in L_R$, i.e., we can accurately estimate the monochromatic degree of each $v_{i'} \in L_R$. So, we can determine the 
  bucket where each vertex in $L_R$ belongs. Let $A_j$ $(=L_R \cap B_j)$ be the bucket $B_j$ projected onto $L_R$.  We determine $\widehat{m_\ell}=\frac{n}{\size{R}}\sum \limits_{j \in [t]}\size{A_j}\left(1+\frac{\vareps}{10}\right)^j$. We can show that $\frac{n}{\size{R}}\size{A_j}$ is a $\left(1+\frac{\vareps}{10}\right)$-approximation of $\size{B_j}$, with high probability, if $\size{B_j}\geq \frac{\sqrt{\vareps T}}{10t}$. Also, we can show that, if $\size{B_j}< \frac{\sqrt{\vareps T}}{10t}$, then 
  $\size{A_j} \leq \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8t}$ with high probability. Now using the fact that we consider bucketing of only low degree vertices($L_R$), we can show that 
  \begin{center}
  \begin{equation}
  \label{eqn:low-over}
   \left(1-\frac{\vareps}{10} \right) \left( m_\ell - \frac{\vareps T}{63t}\right) \leq \widehat{m_\ell} \leq \left(1+\frac{\vareps}{10}\right)^2\left(m_\ell + \frac{\vareps T}{56t} \right).
 \end{equation}
\end{center}
Note that $\vareps \in (0,1)$ and $t=\lceil \log _{1+\frac{\vareps}{10}} n \rceil$. Assuming $T \geq 63t^2$,  Equations~\ref{eqn:high-over} and~\ref{eqn:low-over} imply that $\widehat{m}=\frac{1}{2}(\widehat{m_h} +\widehat{m_\ell})$ is a $(1 \pm \vareps)$-approximation to $\size{E_M}$. If $T < 63t^2$, then note that $n=\widetilde{O}\left(\frac{n}{\sqrt{T}}\right)$. So, in that case, we store all the vertices along with their colors and compute the exact value of $\size{E_M}$. 

\subsection*{Proof of correctness}
The correctness of the algorithm follows trivially if $T < 63t^2$. So, let us assume that $T \geq 63t^2$.
Note that, as $v_1,\ldots,v_n$ arrive in the random order, the first $\widetilde{\Theta}\left( \frac{n}{\sqrt{T}}\right)$ vertices can be thought of as the random sample $R$ without replacement. Using the Chernoff bound for sampling without replacement (See Lemma~\ref{lem:without-replace} in Appendix~\ref{sec:prob}), we can have the following lemma, which will be useful for the correctness proof of the Algorithm~\ref{algo:random-order} ({\sc Random-Order-Est}($\vareps,T)$) in case of $T \geq 63t^2$.
\begin{lem}\label{lem:cher-random-algo}
\begin{itemize}
\item[(i)] For each $j \in [t]$ with $\size{B_j} \geq \frac{\sqrt{\vareps T}}{10t}$, $\pr \left( \size{{\size{B_j \cap R}}-
\frac{\size{R}\size{B_j}}{n}} \geq \frac{\vareps}{10}\frac{\size{R}\size{B_j}}{n}  \right) \leq \frac{1}{n^{10}}$.
\item[(ii)] For each $j \in [t]$ with $\size{B_j} < \frac{\sqrt{\vareps T}}{10t}$, $\mathbb{P} \left( {{\size{B_j \cap R}}} \geq \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8t}  \right) \leq \frac{1}{n^{10}}$.
\item[(iii)] For each vertex $v_i$ with $d_M(v_i) \geq \frac{\sqrt{\vareps T}}{10t}$, $\mathbb{P} \left( \size{\kappa_i - \frac{\size{R}d_M(v_i)}{n}} \geq \frac{\vareps}{10}\frac{\size{R}d_M(v_i)}{n}\right) \leq \frac{1}{n^{10}}$.
\item[(iv)] For each vertex $v_i$ with $d_M(v_i) < \frac{\sqrt{\vareps T}}{10t}$, $\mathbb{P} \left( {\kappa_i} \geq \frac{ \size{R}}{n}\frac{\sqrt{\vareps T}}{8t}\right) \leq \frac{1}{n^{10}}$.
\end{itemize}
\end{lem}

\remove{ Recall that $\widehat{m_h}=\sum\limits_{v_i:\kappa_i \geq \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8t}}\widehat{d_i}$ and $\widehat{m_\ell}=\frac{n}{\size{R}}\sum\limits_{j\in [t]}\size{A_j}\left(1+\frac{\vareps}{10}\right)^{j}$.\\
 Also, $m_h=\sum\limits_{v_i:\kappa_i \geq \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8t}} d_M(v_i)$ and $m_\ell=\sum\limits_{v_i:\kappa_i < \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8t}} d_M(v_i)$. \\
So, $\size{E_M}=\frac{1}{2}(m_h+m_\ell)$. }
The correctness proof of the algorithm is divided into two of the following claims.
\begin{cl}\label{clm:random-high}
$\left(1-\frac{\vareps}{10}\right)m_h\leq \widehat{m_h} \leq \left(1+\frac{\vareps}{10}\right)m_h $ with probability at least $1-\frac{1}{n^{9}}$.
\end{cl}
\begin{cl}\label{clm:random-low}
$\left(1-\frac{\vareps}{10}\right)\left(m_\ell-\frac{\vareps T}{63t}\right) \leq \widehat{m_\ell} \leq \left(1+\frac{\vareps}{10}\right)^2\left(m_\ell+\frac{\vareps T}{56t}\right) $ with probability at least $1-\frac{1}{n^{7}}$. 
\end{cl}
Assuming the above two claims hold and taking $\vareps \in (0,1)$, $t=\lceil \log _{1+\frac{\vareps}{10}} n \rceil$ and $T \geq 63t^2$, observe  that $\widehat{m}=\frac{1}{2}(\widehat{m_h}+\widehat{m_\ell})$ is a $(1\pm \vareps)$ approximation of $\size{E_M}=m_h+m_\ell$ with high probability.
Thus, it remains to prove Claims~\ref{clm:random-high} and~\ref{clm:random-low}.

\begin{proof}[Proof of Claim~\ref{clm:random-high}]
Note that $m_h=\sum\limits_{v_i:\kappa_i \geq \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8t}} d_M(v_i)$ and $\widehat{m_h}=\sum\limits_{v_i:\kappa_i \geq \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8t}}\widehat{d_i}$. 

From Lemma~\ref{lem:cher-random-algo}~(iv) and~(iii), $\kappa_i \geq \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8t}$ implies that $\widehat{d_i}$ is an $\left(1\pm \frac{\vareps}{10}\right)$ approximation to $d_M(v_i)$ with probability at least $1-\frac{2}{n^{10}}$. Hence, we have $\left(1-\frac{\vareps}{10}\right)m_h\leq \widehat{m_h} \leq \left(1+\frac{\vareps}{10}\right)m_h $ with probability at least $1-\frac{1}{n^9}$.
 \end{proof}
 \begin{proof}[Proof of Claim~\ref{clm:random-low}]
 Note that $m_\ell=\sum\limits_{v_i:\kappa_i < \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8t}} d_M(v_i)$ and $\widehat{m_\ell}=\frac{n}{\size{R}}\sum\limits_{j\in [t]}\size{A_j}\left(1+\frac{\vareps}{10}\right)^{j}$.
 Recall that the vertices in $L$ are partitioned into $t$ buckets as follows:\\
$B_j=\{v_i \in L: \left(1+\frac{\vareps}{10} \right)^{j-1} \leq d_M(v_i) < \left(1+\frac{\vareps}{10}\right)^{j} \}$, where $j \in [t]$.
By Lemma~\ref{lem:cher-random-algo}, $\kappa_i < \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8 t}$ implies that $d_M(v_i) \leq \frac{\sqrt{\vareps T}}{7 t}$ with probability $1-\frac{1}{n^{10}}$. So, we have the following observation. 
\begin{obs}\label{obs:low-deg-low-buck}
Let $j \in [t]$ be such that $\size{A_j} \neq 0$ ($\size{B_j}\neq 0$). Then, with probability at least $1-\frac{1}{n^{10}}$, the degree of each vertex in $A_j(B_j)$ is at most $\frac{\sqrt{\vareps T}}{7 t}$, that is, $\left( 1+\frac{\vareps}{10}\right)^{j} \leq \frac{\sqrt{\vareps T}}{7 t}$.
\end{obs}

To upper and lower bound $\widehat{m_\ell}$ in terms of $m_\ell$, we upper and lower bound $m_\ell$ in terms of $\size{B_j}$'s as follows:
\begin{eqnarray*}\label{eqn:exact-low}
&& \sum\limits_{j \in [t]}\size{B_j}\left( 1+\frac{\vareps}{10}\right)^{j-1} \leq  m_\ell  < \sum\limits_{j \in [t]}\size{B_j}\left( 1+\frac{\vareps}{10}\right)^{j} \\
&& \sum\limits_{j \in [t]}\size{B_j}\left( 1+\frac{\vareps}{10}\right)^{j-1} \leq  m_\ell  < \sum\limits_{j \in [t]:\size{B_j}\geq \frac{\sqrt{\vareps T}}{9t}}\size{B_j}\left( 1+\frac{\vareps}{10}\right)^{j} +  \sum\limits_{j \in [t]:\size{B_j}< \frac{\sqrt{\vareps T}}{9t}}\size{B_j}\left( 1+\frac{\vareps}{10}\right)^{j}
 \end{eqnarray*} 
  By Observation~\ref{obs:low-deg-low-buck}, we bound $m_\ell$ in terms of $\size{B_j}$'s with probability $1-\frac{1}{n^9}$.
  \begin{eqnarray*}
 && \sum\limits_{j \in [t]}\size{B_j}\left( 1+\frac{\vareps}{10}\right)^{j-1} \leq  m_\ell  < \sum\limits_{j \in [t]:\size{B_j}\geq \frac{\sqrt{\vareps T}}{9t}}\size{B_j}\left( 1+\frac{\vareps}{10}\right)^{j} +  t \cdot \frac{\sqrt{\vareps T}}{9t}\frac{\sqrt{\vareps T}}{7t}
  \end{eqnarray*}
  This implies the following Observation:
  \begin{obs}\label{obs:exact-low}
$\sum\limits_{j \in [t]}\size{B_j}\left( 1+\frac{\vareps}{10}\right)^{j-1} \leq  m_\ell  < \sum\limits_{j \in [t]:\size{B_j}\geq \frac{\sqrt{\vareps T}}{9t}}\size{B_j}\left( 1+\frac{\vareps}{10}\right)^{j} +  \frac{\vareps T}{63 t}$ holds with probability at least $1-\frac{1}{n^9}$. 
\end{obs}

Now, we have all the ingredients to show that $\widehat{m_\ell}$ is a $(1 \pm \vareps)$ approximation of $m_\ell$. Breaking $ \widehat{m_\ell} = \frac{n}{\size{R}}\sum\limits_{j\in [t]}\size{A_j}\left(1+\frac{\vareps}{10}\right)^{j}$ depending on the value of $\size{A_j}$'s, we  have
 \begin{eqnarray}\label{eqn:low-random}
 \widehat{m_\ell}&=& \frac{n}{\size{R}} \left[\sum\limits_{j\in [t]:\size{A_j} \geq \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8 t}}\size{A_j}
 \left(1+\frac{\vareps}{10}\right)^{j} + \sum\limits_{j\in [t]:\size{A_j} < \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8 t}}\size{A_j}
 \left(1+\frac{\vareps}{10}\right)^{j}\right]
 \end{eqnarray}
 From Lemma~\ref{lem:cher-random-algo}~ (ii) and~(i),  $\size{A_j} \geq \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8 t}$ implies that $\size{A_j}$ is a $\left(1+\frac{\vareps}{10}\right)$-approximation to $\frac{\size{R}\size{B_j}}{n}$ with probability at least $1-\frac{2}{n^{10}}$. 
 \remove{From Lemma~\ref{lem:cher-random-algo}~(i), $\size{A_j} < \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8 t}$ implies that $\size{B_j'}\leq \frac{\sqrt{\vareps T}}{7t}$ with probability at least $1-\frac{1}{n^{10}}$.} 
 From Equation~\ref{eqn:low-random}, we have the following upper bound on $\widehat{m_\ell}$ with probability at least $1-\frac{1}{n^9}$.
 \begin{eqnarray*}
 \widehat{m_\ell} &\leq& 
 \sum\limits_{j\in [t]:\size{A_j} \geq \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8 t}}\left(1+\frac{\vareps}{10}\right)\size{B_j}\left(1+\frac{\vareps}{10}\right)^{j} +
  \sum\limits_{j\in [t]:\size{A_j} < \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8 t}}\frac{\sqrt{\vareps T}}{8t}\left(1+\frac{\vareps}{10}\right)^{j}
  \\
  &\leq & \left(1+\frac{\vareps}{10}\right)^2 \left[ \sum\limits_{j\in [t]:\size{A_j} \geq \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8 t}}\size{B_j}\left(1+\frac{\vareps}{10}\right)^{j-1} +   \sum\limits_{j\in [t]:\size{A_j} < \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8 t}}\frac{\sqrt{\vareps T}}{8t}\left(1+\frac{\vareps}{10}\right)^{j-1}
 \right]
 \end{eqnarray*}
 Now by Observations~\ref{obs:exact-low} and ~\ref{obs:low-deg-low-buck}, we have the following with probability at least $1-\frac{1}{n^8}$.
 \begin{eqnarray*}
 \widehat{m_\ell} &\leq& \left(1+\frac{\vareps}{10}\right)^2 \left( m_\ell + t \cdot \frac{\sqrt{\vareps T}}{8t}\frac{\sqrt{\vareps T}}{7t}\right) \\
 &=&  \left(1+\frac{\vareps}{10}\right)^2 \left( m_\ell + \frac{\vareps T}{56 t}\right)
 \end{eqnarray*}
 Now, we will lower bound $\widehat{m_\ell}$. From Equation~\ref{eqn:exact-low}, we have 
 \begin{eqnarray*}
 \widehat{m_\ell} &\geq& \frac{n}{\size{R}} \sum\limits_{j\in [t]:\size{A_j} \geq \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8 t}}\size{A_j}
 \left(1+\frac{\vareps}{10}\right)^{j} 
 \end{eqnarray*}
 Once again note that, from Lemma~\ref{lem:cher-random-algo}~(i) and~(ii),  $\size{A_j} \geq \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8 t}$ implies $\size{A_j}$ is a $\left(1+\frac{\vareps}{10}\right)$-approximation to $\frac{\size{R}\size{B_j}}{n}$ with probability at least $1-\frac{2}{n^{10}}$. So, the following holds with probability $1-\frac{1}{n^{9}}$.
   \begin{eqnarray*}
 \widehat{m_\ell} &\geq& \left(1-\frac{\vareps}{10} \right) \sum\limits_{j\in [t]:\size{A_j} \geq \frac{\size{R}}{n}\frac{\sqrt{\vareps T}}{8 t}}\size{B_j}
 \left(1+\frac{\vareps}{10}\right)^{j} 
 \end{eqnarray*}
By Lemma~\ref{lem:cher-random-algo}~(i), if $\size{B_j} \geq \frac{\sqrt{\vareps T}}{9t}$, then $\size{A_j} \geq \frac{\sqrt{\vareps T}}{8t}$ with probability at least $1-\frac{1}{n^{10}}$. Hence, we have the following lower bound on $m_\ell$ with probability at least $1-\frac{1}{n^8}$.

 \begin{eqnarray*}
\widehat{m_\ell} &\geq& \left(1-\frac{\vareps}{10} \right) \sum\limits_{j\in [t]:\size{B_j} \geq {\frac{\sqrt{\vareps T}}{9 t}}}\size{B_j}
 \left(1+\frac{\vareps}{10}\right)^{j} 
 \end{eqnarray*}
 Now by Observation~\ref{obs:exact-low}, we have the following with high probability at least $1-\frac{1}{n^7}$.
 \begin{eqnarray*}
 \widehat{m_\ell} &\geq &  \left(1-\frac{\vareps}{10} \right) \left( m_\ell - \frac{\vareps T}{63t}\right).
 \end{eqnarray*}

\end{proof}
























==> temp-tech-gopi.tex <==
\section{\conflictest in arbitrary order \va and \vadeg models}\label{sec:est-vaubsc}
 
The \conflictest problem in streaming asks to approximately estimate the number of monochromatic edges, $\size{E_M}$, in a graph arriving in a streaming manner. In this section we design algorithms for this problem in the vertex arrival model of streaming. We show later that the bounds obtained in the vertex arrival model are tight. Hence, we look at two variants of the vertex arrival model. In one such model we assume access to a \emph{degree oracle} and in the other model, we assume a random order of vertices. For this discussion below, we assume a lower bound $T$ on the number of monochromatic edges in the graph. 
% \comments{Anup: $T$ need not be given to us explicitly. Using binary search we should be able to obtain $\Tilde{T}$ which is within a factor of $2$ of $T$ using $O(\log n)$ space overhead. In the remainder of this paper, we assume $T$ is given.}
 
% \subsection{\conflictest in \vadeglong and arbitrary order \valong model}\label{sec:est-vadeg3}

In this section we design an algorithm for estimating the number of monochromatic edges in a graph appearing over a stream in the vertex arrival model with degree oracle. In addition, we assume access to a degree oracle $d_G: V\rightarrow \mathbb{R}_+$ that returns the degree of a vertex. We will give a $\widetilde{\mathcal{O}} \left(\frac{m}{T} \right)$ space streaming algorithm for estimating the number of monochromatic edges.

The main idea is to sample $\widetilde{\mathcal{O}} \left(\frac{m}{T} \right)$ edges uniformly at random from the stream along with their colors and count the number of monochromatic edges. To sample a uniform edge, we do the following. For any vertex $v$ in the stream, we query for $d_G(v)$ and store that vertex along with its color using a weighted reservoir sampler with weight $d^{+}_G(v)$, where $d^{+}_G(v)$ denotes the number of neighbours of $v$ to its right\footnote{$d^{+}_G(v)$ is obtained by subtracting the number of edges from $v$ to the vertices exposed earlier from $d_G(v)$.}. We also sample a number $j\in [d^{+}_G(v)]$ uniformly at random. We keep track of the number of neighbours of $v$ that appears after $v$ in the stream such that we store edge $(v,w)$, where $w$ is the $j\in [d^{+}_G(v)]$th neighbour of $v$. Notice that $(v,w)$ is a uniformly sampled edge from the stream. We maintain $\widetilde{\mathcal{O}} \left(\frac{m}{T} \right)$ such edges using $\widetilde{\mathcal{O}} \left(\frac{m}{T} \right)$ weighted reservoir samplers.

%To estimate the number of monochromatic edges, $\size{E_M}$, in the \vadeg model, we uniformly sample a subset of $\widetilde{\mathcal{O}} \left(\frac{m}{T} \right)$ vertex pairs and their colors \footnote{Using reservoir sampling}. When a vertex $u$ arrives in the stream, we store $u$ and its color, if it is sampled. We then store the $j^{th}$ neighbor of $u$ appearing to its right in the stream, where $j \in \left[ d^{+}_{G} \left(u \right) \right]$. Since we have access to a degree oracle, we know $d_{G} \left(u \right)$ and can compute $d^{+}_{G} \left(u \right)$ using this information. When we encounter the $j^{th}$ neighbor of $u$ later in stream, we check the edge for conflict. The number of edges effectively sampled is $\widetilde{\mathcal{O}} \left(\frac{m}{T} \right)$, each of them independently and uniformly at random with probability $\widetilde{\mathcal{O}} \left(\frac{1}{T} \right)$. We check each of the sampled edges for conflict and using this count, estimate the total number of monochromatic edges in the graph.

\begin{theorem}\label{theo:est-vadgubth}
Given any graph $G=(V,E)$ and a coloring function $f: V(G) \rightarrow [C]$ as input in the stream, there exists an algorithm that solves the \conflictest problem in the \vadeg streaming model with high probability in $\widetilde{\mathcal{O}} \left(\frac{m}{T} \right)$ space, where $T$ is a lower bound on the number of monochromatic edges in the graph.  \end{theorem}
 
\begin{proof} Let us sample $t=\frac{2m}{\eps^2 T}\log n$ edges uniformly at random from the stream and for each edge, check if it is monochromatic or not. Let $X_i$ denote an indicator random variable that equals one if the $i$th sampled edge is monochromatic, zero otherwise. Let our estimator be $\Tilde{Y}=\frac{m}{t} \sum_{i=1}^t X_i$. The expected value of the estimator $\E[\Tilde{Y}]=Y$, where $Y$ denotes the number of monochromatic edges in the graph. Note that multiplying by $m$ is fine because we do this at the end of the stream when we know $m$.

Let $X=\sum_{i=1}^t X_i$. Since $t=\frac{2m}{\eps^2 T}\log n$, we have $\E[X]=t \frac{Y}{m}\geq 2\log n$. Using Chernoff bounds, with probability at least $(1-1/n^2)$, we have $(1-\eps)\E[X]\leq X\leq (1+\eps) \E[X]$. Therefore, with probability at least $(1-1/n^2)$, $(1-\eps)Y\leq \Tilde{Y}\leq (1+\eps)Y$.


%We sample a vertex $u$ and its color $f(u)$ in the stream.
%\[  \mathcal{P}(\texttt{an edge e is conflicting}) \geq \frac{T}{m}   \]
%If we sample $t$ edges overall, independently and uniformly at random, then,
%\[  \mathcal{P}(\texttt{none of the edges sampled are conflicting}) \leq \left(1-\frac{T}{m} \right)^t \leq e^{-\frac{Tt}{m}}  \] 
%In effect, we check $\widetilde{\mathcal{O}} \left(\frac{m}{T} \right)$ edges for conflict. Let $S$ be the number of monochromatic edges in the sample of edges selected and let $C$ be the total number of monochromatic edges in the graph. We assume an ordering of the monochromatic edges in the graph. To estimate the number of monochromatic edges in the graph, we do the following:
%Let $S_{i}$ be an indicator random variable defined as follows:
 %[  S_{i} = \left\{
 %       \begin{array}{ll}
 %           1 & \quad \text{if the } i^{th} \text{ monochromatic edge is sampled with probability } \widetilde{\mathcal{O}}\left(\frac{1}{T}\right) \\
 %           0 & \quad \text{otherwise}
 %       \end{array}
 %   \right.
%\] 
 %$S = \sum S_{i}$
 %\[  \mathbb{E} [S] = \mathbb{E} \left[ \sum S_{i} \right] = \sum \mathbb{E} \left[S_{i} \right] = \sum \frac{k \log n}{T} = \frac{k C \log n}{T}  \]
%for some constant $k$.

%Thus, the expected number of monochromatic edges in the sample is $\mathbb{E} [S]= \frac{k C \log n}{T} $.  The algorithm calculates the sample size $S$ and reports the number of monochromatic edges in the graph as $C^{'}$, where $C^{'} = \frac{k^{'} S T}{\log n}$ for some constant $k^{'}$ and $\mathbb{E} [C^{'}] = C$.
 %\[  \mathcal{P} \left(\size{C' - C} \geq \vareps C \right) = \mathcal{P} \left(\size{S - \frac{10C \log n}{\vareps^{2}T}} \geq \frac{10 C \log n}{\vareps T} \right)   \]
 %Applying Chernoff bound [Lemma~\ref{lem:cher_bound1}], we get:
 %\[  \mathcal{P}\left(\size{S - \frac{10C \log n}{\vareps^{2}T}} \geq \frac{10 C \log n}{\vareps T} \right) \leq 2 \exp \left(-\frac{10 C \log n}{\vareps^{2}T}\frac{\vareps^{2}}{3} \right) \leq 2n^{-3}   \]
 %since $C > T$.
 
 %With high probability, we can solve the \conflictest problem in $\widetilde{\mathcal{O}} \left(\frac{m}{T} \right)$ space in the \vadeg model.
 \end{proof}
 
 %%%%%
 \comments{Anannya: Initial write-up start}

To estimate the number of monochromatic edges in the \vadeg model, we uniformly sample a subset of $\widetilde{\mathcal{O}} \left(\frac{m}{T} \right)$ vertex pairs and their colors \footnote{Using reservoir sampling}. When a vertex $u$ arrives in the stream, we store $u$ and its color, if it is sampled. We then store the $j^{th}$ neighbor of $u$ appearing to its right in the stream, where $j \in \left[ d^{+}_{G} \left(u \right) \right]$. Since we have access to a degree oracle, we know $d_{G} \left(u \right)$ and can compute $d^{+}_{G} \left(u \right)$ using this information. When we encounter the $j^{th}$ neighbor of $u$ later in stream, we check the edge for conflict. The number of edges effectively sampled is $\widetilde{\mathcal{O}} \left(\frac{m}{T} \right)$, each of them independently and uniformly at random with probability $\widetilde{\mathcal{O}} \left(\frac{1}{T} \right)$. We check each of the sampled edges for conflict and using this count, estimate the total number of monochromatic edges in the graph.

\begin{theorem} Given an input graph $G = (V, E)$, a coloring function $f : V(G) \rightarrow [C]$, we can solve the \conflictest problem in the \vadeg streaming model with high probability in $\widetilde{\mathcal{O}} \left(\frac{m}{T} \right)$ space, where $T$ is a lower bound on the number of monochromatic edges in the graph.  \end{theorem}
 
\begin{proof}
We sample a vertex $u$ and its color $f(u)$ in the stream.
\[
 \mathcal{P}(\texttt{an edge e is conflicting}) \geq \frac{T}{m} 
 \]
 If we sample $t$ edges overall, independently and uniformly at random, then,
 \[
 \mathcal{P}(\texttt{none of the edges sampled are conflicting}) \leq \left(1-\frac{T}{m} \right)^t \leq e^{-\frac{Tt}{m}}
 \] 
In effect, we check $\widetilde{\mathcal{O}} \left(\frac{m}{T} \right)$ edges for conflict. Let $S$ be the number of monochromatic edges in the sample of edges selected and let $C$ be the total number of monochromatic edges in the graph. We assume an ordering of the monochromatic edges in the graph. To estimate the number of monochromatic edges in the graph, we do the following:
Let $S_{i}$ be an indicator random variable defined as follows:
 \[
 S_{i} = \left\{
        \begin{array}{ll}
            1 & \quad \text{if the } i^{th} \text{ monochromatic edge is sampled with probability } \widetilde{\mathcal{O}}\left(\frac{1}{T}\right) \\
            0 & \quad \text{otherwise}
        \end{array}
    \right.
\] 
 $S = \sum S_{i}$
 \[
 \mathbb{E} [S] = \mathbb{E} \left[ \sum S_{i} \right] = \sum \mathbb{E} \left[S_{i} \right] = \sum \frac{k \log n}{T} = \frac{k C \log n}{T}
 \]
for some constant $k$.

Thus, the expected number of monochromatic edges in the sample is $\mathbb{E} [S]= \frac{k C \log n}{T} $.
 The algorithm calculates the sample size $S$ and reports the number of monochromatic edges in the graph as $C^{'}$, where $C^{'} = \frac{k^{'} S T}{\log n}$ for some constant $k^{'}$ and $\mathbb{E} [C^{'}] = C$.
 \[
 \mathcal{P} \left(\size{C' - C} \geq \vareps C \right) = \mathcal{P} \left(\size{S - \frac{10C \log n}{\vareps^{2}T}} \geq \frac{10 C \log n}{\vareps T} \right) 
  \]
 Applying Chernoff bound [Lemma~\ref{lem:cher_bound1}], we get:
 \[
 \mathcal{P}\left(\size{S - \frac{10C \log n}{\vareps^{2}T}} \geq \frac{10 C \log n}{\vareps T} \right) \leq 2 \exp \left(-\frac{10 C \log n}{\vareps^{2}T}\frac{\vareps^{2}}{3} \right) \leq 2n^{-3}
  \]
 since $C > T$.
 
 With high probability, we can solve the \conflictest problem in $\widetilde{\mathcal{O}} \left(\frac{m}{T} \right)$ space in the \vadeg model.
 \end{proof}
  \comments{Anannya: Initial write-up end}
 %%%%%%
 
\begin{remark}
The above result also holds in the \allong model.
\end{remark}

The algorithm in the arbitrary order vertex arrival model is an extension of the algorithm in the vertex arrival model with degree oracle.
 \begin{coro}
 Given any graph $G=(V,E)$ and a coloring function $f: V(G) \rightarrow [C]$ as input in the stream, there exists an algorithm that solves the \conflictest problem in the arbitrary order \va streaming model with high probability in $\widetilde{\mathcal{O}} \left( \min \left( \size{V},\frac{|V|^2}{T} \right) \right) $ space, where $T$ is a lower bound on the number of monochromatic edges in the graph. 
 \end{coro}
 We explicitly mention our results in Appendix~\ref{sec:est-vaaoubsc}.

\input{random.tex}


==> temp-tech.tex <==
\section{\conflictest in \va and \vadeg models}\label{sec:est-vaubsc}

 
\remove{The \conflictest problem in streaming asks to approximately estimate the number of monochromatic edges, $\size{E_M}$, in a graph arriving in a streaming manner.} In this Section, we design algorithms for \conflictest problem in the \va and \vadeg models. We show later the matching lower bounds in Section~\ref{sec:est-lowerbound}. Mainly, we prove the following two theorems. \remove{in sections~\ref{theo:est-vaubth} in Section~\ref{sec:ub-vadeg} and~\ref{sec:ub-arbit}, respectively.}

 \begin{theorem}\label{theo:est-vaubth}
 Given any graph $G=(V,E)$ and a coloring function $f: V(G) \rightarrow [C]$ as input in the stream, there exists an algorithm that solves the \conflictest problem in the \va model with high probability in $\widetilde{\mathcal{O}} \left( \min \left( \size{V},\frac{|V|^2}{T} \right) \right) $ space, where $T$ is a lower bound on the number of monochromatic edges in the graph. 
 \end{theorem}
\begin{theorem}\label{theo:est-vadgubth}
Given any graph $G=(V,E)$ and a coloring function $f: V(G) \rightarrow [C]$ as input in the stream, there exists an algorithm that solves the \conflictest problem in the \vadeg model with high probability in $\widetilde{O}\left(\min\{\size{V}, \frac{\size{E}}{T}\}\right)$ space, where $T$ is a lower bound on the number of monochromatic edges in the graph.  \end{theorem}

Before going to the algorithms for \conflictest problem in the \va and \vadeg model, we would like to discuss as a warm-up, a two pass algorithm for \conflictest in \va model that uses $\widetilde{O}\left(\min\{\size{V}, \frac{\size{E}}{T}\}\right)$ space, where $T$ is the number of edges in the graph and $T$ is the promised lower bound on the number of monochromatic edges in the graph. Moreover, we are assuming that the number of edges is known apriori, in this case, for simplicity of exposition. However, this assumption can be removed by a simple tweak.
\paragraph*{A two-pass algorithm for \conflictest in \va model (Informal):} 
\begin{description}
\item[If $T \leq \frac{\size{E}}{\size{V}}$:] Equivalently, we can check if $T<V$ since $\frac{\size{E}}{\size{V}} < V$. Our algorithm stores all the vertices and their colors. Thus we can determine the number of monochromatic edges exactly. The algorithm in this case is one pass and uses $\widetilde{O}(\size{V})$ space.
\item[If $T > \frac{\size{E}}{\size{V}}$:] In the first pass, store each edge with probability $\widetilde{O}\left(\frac{1}{T}\right)$. In the second pass, we check each edge stored in the first pass for conflict. In this way, we determine the number of monochromatic edges in the sample, from which, we can obtain a desired approximation of the number of monochromatic edges in the graph. The space complexity of our algorithm in this case is $\widetilde{O}\left( \frac{\size{E}}{T}\right)$.
\end{description} 
If only one pass is allowed, the above algorithm, when $T>\frac{\size{E}}{\size{V}}$, can not be simulated in \va model because of the following reason. Consider an edge $(u,v) \in E_M$ such that $u$ is exposed before $v$. Note that we will be able to know about the edge only when $v$ is exposed but we will be able to check whether $(u,v) \in E_M$ only when we have stored $u$ and its color. However, there is no clue about the edge $(u,v)$ when $u$ is exposed. So, to solve it in one-pass, we sample each pair of vertices with probability $\widetilde{O}\left( \frac{1}{T}\right)$, before the start of the stream, and determine the number of monochromatic edges in the sample to get an estimate of the number of monochromatic edges in $G$. This implies that the space complexity of the algorithm for \conflictest in \va model is $\widetilde{O}\left( \frac{\size{V}^2}{T}\right)$ as stated in Theorem~\ref{theo:est-vaubth}. In \vadeg model, when $u$ is exposed we will get $d_G(u)$ and hence $d^+_G(u)$. The degree information, when $u$ is exposed, gives some statistics regarding how the vertex $u$ might be useful in the future. We exploit this advantage of \vadeg model over \va model to get an algorithm for \conflictest that has better space complexity (See Theorem~\ref{theo:est-vadgubth}).

\subsection{Proof of Theorem~\ref{theo:est-vaubth}}\label{sec:ub-vadeg}
Our algorithm for \conflictest for \va model, first checks if $T \leq \frac{\size{E}}{\size{V}}$. If yes, we store all the vertices along with their colors to estimate the number of monochromatic edges in the graph exactly. So, the space used by the algorithm is $\widetilde{O}(\size{V})$ when $T \leq \frac{\size{E}}{\size{V}}$. We will be done by giving an algorithm for \conflictest in \va model that uses $\widetilde{O}\left( \frac{\size{V}^2}{T}\right)$ space. This algorithm will only be executed when $T > \frac{\size{E}}{\size{V}}$.
 
Let $V=\{v_1,\ldots,v_n\}$ be the vertices of the graph. Our algorithm starts by generating a sample $Z$ of vertex pairs where each $\{v_i,v_j\}$ is added to $Z$, independently, with probability $\frac{30 \log n}{\eps^2 T}$. Note that $Z$ is obtained before the start of the stream. Over the stream, we check the following for each $\{v_i,v_j\}\in Z$: whether $(v_i,v_j) \in E$ and is monochromatic.
\remove{
\begin{itemize}
\item whether $(v_i,v_j)$ is an edge,
\item whether $f(v_i)=f(v_j)$, that is, whether $(v_i,v_j)$ is a monochromatic edge.
\end{itemize}
}
Let $S \subseteq Z$ be the set of monochromatic edges in $Z$. Note that the expected value of $\size{S}$ is  given by $\E[\size{S}]=\frac{30 \log n}{\eps^2 T}\size{E_M}$.

We report $\widehat{m}=\frac{\eps^2 T}{30 \log n}\size{S}$ as our estimate for $\size{E_M}$. Applying Chernoff bound (See Lemma~\ref{lem:cher_bound1} in Appendix~\ref{sec:prob}), we guarantee that 
$$\pr \left(\size{\widehat{m}-\size{E_M}} \geq \eps \size{E_M}\right)\leq \pr \left(\size{\size{S}-\E[\size{S}]} \geq \eps \E[\size{S}]\right) \leq \exp{\left(\frac{-\E[\size{S}]\eps^2}{3}\right)}\leq \frac{1}{n^{10}}.$$
Note that the last inequality holds as $\E[\size{S}]=\frac{30 \log n}{\eps^2 T}\size{E_M}$ and $\size{E_M}\geq T$.

Observe that the space used by our algorithm is $O(\size{Z})$ when $T > \frac{\size{E}}{\size{V}}$. Note that $\E[\size{Z}]=\frac{30 \log n}{\eps^2 T}{n \choose 2}$. Applying Chernoff bound (See Lemma~\ref{lem:cher_bound1} in Appendix~\ref{sec:prob}), we can show that $\size{Z}=\widetilde{O}\left( \frac{n^2}{T}\right)$ with high probability.

Putting together the space complexities of our algorithms for the case $T \leq \frac{\size{E}}{\size{V}}$ and $T > \frac{\size{E}}{\size{V}}$, we have the desired bound on the space.
\subsection{Proof of Theorem~\ref{theo:est-vadgubth}}\label{sec:ub-arbit}
 Our algorithm for \conflictest for \vadeg model, first checks if $T \leq \frac{\size{E}}{\size{V}}$, similar to the algorithm for \conflictest in \va model. If yes, we store all the vertices along with their colors to estimate the number of monochromatic edges in the graph exactly. So, the space used by the algorithm is $\widetilde{O}(\size{V})$ when $T \leq \frac{\size{E}}{\size{V}}$. We will be done by giving an algorithm for \conflictest in \vadeg model that uses $\widetilde{O}\left(\frac{\size{E}}{T}\right)$ space. This algorithm will only be executed when $T > \frac{\size{E}}{\size{V}}$.
 
Let $V=\{v_1,\ldots,v_n\}$ and w.o.l.g. the vertices are exposed in the order $v_1,\ldots,v_n$. However, our algorithm does not know about the ordering of the vertices. Our algorithm stores the following information.
\begin{itemize}
\item  A random subset set $Y \subset V \times [n]$ that will be generated over the stream;
\item  a subset $A$ of vertices present as the first element in the pairs present in $Y$ along with their colors;
\item  for each vertex $v \in A$, the number $\ell_v$ that denotes the number of neighbors in $N_G^+(v)$;
\item a subset $S\subseteq E_M$ of the set of monochromatic edges in $G$.
\end{itemize}
When a vertex $v_j$ is exposed, our algorithm performs the following steps:
\begin{itemize}
\remove{\item[(i)] Set $d^-_G(v_j)$ equals to the number of neighbors that $v_j$ has in $\{v_1,\ldots,v_{j-1}\}$. Get $d_G(v_j)$ from 
the degree oracle and compute $d_G^+(v_j)$;}
\item[(i)] Get $d_G(v_j)$ from the degree oracle and $d_G^-(v_j)$ from the exposed edges and compute $d_G^+(v_j)$;
\item[(ii)] Add $(v_j,k), k\in \left[d_G^+(v_j)\right]$, with probability $\frac{30 \log n}{\eps^2 T}$ to $Y$, independently; 
\item[(iii)] For each $v_i \in A$ such that $(v_i,v_j) \in E(G)$, increment $\ell_{v_i}$ by $1$. 
\item[(iv)] If for $v_i \in A$ such that $(v_i,\ell_{v_i}) \in Y$, check whether $(v_i,v_j)$ is monochromatic. If yes, add $(v_i,v_j)$ to $S$.  
\item[(v)] Add $v_j$ to $A$ if at least one  $(v_j,k)$ is added to $Y$.
\end{itemize}
The main catch of the algorithm for \conflictest in \vadeg model is in Step-(ii). Due to the added power of degree oracle, we are able to sample edges that have not arrived explicitly in the stream. We refer to this phenomenon as \emph{sampling into the future} in Section~\ref{sec:ideas}.
 
At the end of the stream, we report $\widehat{m}=\frac{\eps^2 T}{30 \log n}\size{S}$ as the estimate of $\size{E_M}$. Now, we show that 
$\pr\left(\size{\hat{m}-\size{E_M}}\geq \eps \size{E_M}\right) \leq \frac{1}{n^{10}}.$
Consider a monochromatic edge $(v_i,v_j)\in E_M$. Let $r \in \left[d_G^+(u)\right]$ be such that $u$ has $r-1$ many neighbors in $\{v_{i+1},\ldots,v_{j-1}\}$. So, $v_j$ is the $r$-th neighbor of $u$ exposed after the exposure of $v_i$. From the description of the algorithm, $(v_i,v_j)$ is added to $S$ if and only if $(v_i,r)$ is added to $Y$.  Note that $(v_i,r)$ can only be added to $Y$ only when the vertex $v_i$ is exposed in the stream. So, the probability that a monochromatic edge is added to $S$ is $\frac{30 \log n}{\eps^2 T}$. That is, $\E[\size{S}]=\frac{30 \log n}{\eps^2 T} \size{E_M}$. Applying Chernoff bound (See Lemma~\ref{lem:cher_bound1} in Appendix~\ref{sec:prob}), we can guarantee that 
$$\pr \left(\size{\widehat{m}-\size{E_M}} \geq \eps \size{E_M}\right)\leq \pr \left(\size{\size{S}-\E[\size{S}]} \geq \eps \E[\size{S}]\right) \leq \exp{\left(\frac{-\E[\size{S}]\eps^2}{3}\right)}\leq \frac{1}{n^{10}}.$$
Note that the last inequality holds as $\size{E_M} \geq T$.
Observe that the space used by the algorithm is $\widetilde{O}(\size{Y}+\size{A}+\size{S})=\widetilde{O}({\size{Y}})$. Note that $\E[\size{Y}]=\sum\limits_{i=1}^n d_G^+(v_i)\cdot \frac{30 \log n}{\eps^2 T}=\frac{30 \size{E}\log n}{\eps^2 T}$. Applying Chernoff bound (See Lemma~\ref{lem:cher_bound1} in Appendix~\ref{sec:prob}), we can say that $\size{Y}=\widetilde{O}\left( \frac{\size{E}}{T}\right)$ with high probability.

Putting together the space complexities of our algorithms for the case $T \leq \frac{\size{E}}{\size{V}}$ and $T > \frac{\size{E}}{\size{V}}$, we have the desired bound on the space.
\input{random.tex}

